Embedding Code Contexts for Cryptographic API Suggestion:New Methodologies and Comparisons

Despite recent research efforts, the vision of automatic code generation through API recommendation has not been realized. Accuracy and expressiveness challenges of API recommendation needs to be systematically addressed. We present a new neural network-based approach, Multi-HyLSTM for API recommendation --targeting cryptography-related code. Multi-HyLSTM leverages program analysis to guide the API embedding and recommendation. By analyzing the data dependence paths of API methods, we train embedding and specialize a multi-path neural network architecture for API recommendation tasks that accurately predict the next API method call. We address two previously unreported programming language-specific challenges, differentiating functionally similar APIs and capturing low-frequency long-range influences. Our results confirm the effectiveness of our design choices, including program-analysis-guided embedding, multi-path code suggestion architecture, and low-frequency long-range-enhanced sequence learning, with high accuracy on top-1 recommendations. We achieve a top-1 accuracy of 91.41% compared with 77.44% from the state-of-the-art tool SLANG. In an analysis of 245 test cases, compared with the commercial tool Codota, we achieve a top-1 recommendation accuracy of 88.98%, which is significantly better than Codota's accuracy of 64.90%. We publish our data and code as a large Java cryptographic code dataset.

==> Comprehensive Comparisons of Code Embedding Methodologies for Java Cryptographic Applicatons/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> Comprehensive Comparisons of Code Embedding Methodologies for Java Cryptographic Applicatons/Sections/1-introduction.tex <==

\section{Introduction}

%[Problem stated]
%An API recommendation tool can be useful to assist developers and provide the semi-automatic code generation.  the code completion can be a good support for dev  code involving complex APIs. Given an incomplete code snippet, the API likely to be used are recommended as a ranked list. Many studies show that intelligent API recommendation plugins based on the statistical or deep learning approaches achieve good top-k accuracy on the API recommendation. However, that  

%Modern software makes heavy use of standard or third-party libraries, making understanding the API usage important to many software engineering tasks, including API misuse detection, code repair, and API suggestion, etc. Learning the correct usage of the countless APIs is not easy for developers. Multiple studies have shown that misusing Java cryptographic APIs introduces vulnerabilities~\cite{egele2013empirical,rahaman2019cryptoguard,kruger2017cognicrypt}. In addition, studies showed that the misuses of Java cryptographic APIs are common in practice~\cite{meng2018secure,votipka2020understanding,acar2016you}, which is partly due to API complexity and insufficient documentation~\cite{kruger2017cognicrypt}. Misleading insecure code snippets on popular online forums (e.g. StackOverflow) worsen the situation~\cite{meng2018secure,chen2019reliable}. An API recommendation tool that gives accurate suggestion for the next API method call based on the previous code can be helpful and contributes to semi-automatic code generation.
Modern software relies heavily on standard or third-party libraries. However, learning the correct usage of countless APIs is challenging for developers due to API complexity and insufficient documentation~\cite{kruger2017cognicrypt}, and often leads to misuse of APIs~\cite{meng2018secure, votipka2020understanding, acar2016you}. For example, multiple studies have shown that misusing Java cryptographic APIs is common in practice~\cite{egele2013empirical,rahaman2019cryptoguard,chen2019reliable}. Thus, a tool suggesting correct API methods would help developers from misuse.

%State-of-the-art API recommendation solutions typically utilize machine learning models with program analysis~\cite{raychev2014code,nguyen2016learning,nguyen2016api,svyatkovskiy2019pythia}. Statistical language models (LMs) are trained with the sequences extracted via static analysis to produce recommendations. For example, SLANG~\cite{raychev2014code} leverages the recurrent neural network (RNN) and $n$-gram model to learn the extracted method call sequences associated with an object. SALAD~\cite{nguyen2016learning} introduces the hidden Markov model of API usage (HAPI) to learn the API method call sequences extracted from a graph based object usage model (GROUM)~\cite{nguyen2009graph}. Given previous code lines, the tools produce a ranked candidate list based on the probabilities calculated by the machine learning model.  Despite the significant progress, there is still room for improving prediction accuracy, especially for the critical APIs and  complex APIs. Existing solutions show good top-{\em k} accuracy, however, it may still be difficult for developers to select the correct API method from the list. 
Despite the significant progress in suggesting the next API(s), there is still room for improving prediction accuracy, especially for critical and complex APIs. Most state-of-the-art API recommendation solutions~\cite{raychev2014code, nguyen2016learning, nguyen2016api, svyatkovskiy2019pythia,nguyen2020code} utilize machine learning models with program analysis and suggest top-{\em k} APIs. 
%Existing solutions show good top-{\em k} accuracy in terms of suggesting top-{\em k} APIs, 
%However, it may still be difficult for developers to select the correct API method from the top-{\em k} API list. Besides, leveraging neural network models with proper program analysis is the key to precise API recommendation. 
%\fixme{The following blue-colored text should go to the related work section}. \textcolor{blue}{Statistical language models (LMs) are trained with the sequences extracted via static analysis to produce recommendations. For example, SLANG~\cite{raychev2014code} leverages the recurrent neural network (RNN) and $n$-gram model to learn the extracted method call sequences associated with an object. SALAD~\cite{nguyen2016learning} introduces the hidden Markov model of API usage (HAPI) to learn the API method call sequences extracted from a graph-based object usage model (GROUM)~\cite{nguyen2009graph}. Given previous code lines, the tools produce a ranked candidate list based on the probabilities calculated by the machine learning model.}
We aim to design reliable API method recommendation approaches with high \textbf{top-1 accuracy}, as well as comprehensively compare the accuracy capabilities of multiple program analysis and programming language modeling methodologies. %\fixme{Need to discuss the general applicability of the approach and reason for choosing Java crypto APIs.}

Making accurate recommendations on API method calls is challenging due to several reasons. \textit{First}, the programming context necessary to make a precise recommendation is often missing. In real-world codebases, many essential code dependencies often locate in other methods or files far away from the places of recommendation queries. Source code sequences, abstract syntax trees (ASTs), and \textit{intraprocedural} static analysis traces~\cite{raychev2014code,hindle2012naturalness,ray2016naturalness,chen2019sequencer} are likely to miss them due to the insufficient coverage beyond the local method. 
%Meanwhile, it may be challenging to extend the intraprocedural code context to interprocedural ones due to the dramatically increased size and complexity. 



\textit{Second}, neural network models need to be specialized to address programming language-specific challenges. For example, we find that existing sequence models (e.g., LSTM) only capture the most frequent API sequence patterns. There are many low-frequency patterns that are neglected. This issue is more severe when a less frequent pattern shares a common suffix with a high-frequency one (Figure~\ref{fig:example_frequency} (a)). This shared segment misleads LSTM to make a wrong prediction.  
%For example,  Fig.~\ref{fig:global_influence_example} (a) shows a common pattern (dependence chain of API method calls) while Fig.~\ref{fig:global_influence_example} (b) shows a slightly different dependence path that is rarer. Recognizing Fig.~\ref{fig:global_influence_example} (b) is difficult because it is too similar to (a) while suggesting a different next API method. 
Recent Transformer models that use an attention mechanism~\cite{vaswani2017attention,devlin2018bert} to identify important parts of the input sequence, do not solve the frequency imbalance problem as well.
%Although the attention mechanism of the transformer model~\cite{vaswani2017attention,devlin2018bert} treats the input tokens parallel, thus can recognize which parts of the input sequence are important. However, the challenge posed by frequency imbalance is still not solved. 
%To address this issue, we develop a neural network model called HyLSTM a low-frequency long-range enhancing technique called HyLSTM that is capable of recognizing low-frequency patterns.      
%To address this issue, we develop a low-frequency long-range enhancing technique called HyLSTM that is capable of recognizing low-frequency patterns.      

%as well as being resistant against differences caused by noise. That is inherently conflicting for the deep learning models without any preliminary knowledge. 




\sloppy{
%Third, some functionally-similar API methods are difficult to differentiate due to their similar programming context. For example, both \lstinline|new String(byte[])| and \lstinline|Base64.Encoder.encodeToString(byte[])| are possible used after \lstinline|Cipher| decryption to convert the decrypted \lstinline|byte[]| to a \lstinline|String|.  There is no indicator from the former \lstinline|Cipher| decryption operations to tell which one to use. 
%For example, both \verb|Cipher.init(int, Key)| and \verb|Cipher.init(int, Key, AlgorithmParameterSpec)| initialize the \verb|Cipher| instance. 
%However, they are not interchangeable in codebase~\fixme{due to what?}.\footnote{In contrast, synonyms are usually interchangeable in natural language settings.} It is decided by an earlier dependence happened to the data, the API method used to covert the original \lstinline|String| to \lstinline|byte[]| before the encryption. Only capturing both of the dependence paths for the \lstinline|Cipher| operations and the data processing operations can tell the accurate API method. Therefore, we increase our recommendation accuracy by aggregating multiple dependence paths to increase the coverage for different dependencies. 
\textit{Third}, another programming language-specific challenge is differentiating between functionally-similar, but non-interchangeable API methods.
%Third, some API methods are difficult to differentiate due to their similar but non-interchangeable programming behaviors. 
%The correct API suggestion from a set of functionally-similar APIs requires a dependence analysis of the parameters passed to these APIs. 
For example, \lstinline|new String(byte[])| and \lstinline|Base64.Encoder.encodeToString(byte[])| are two candidate APIs after \lstinline|Cipher| decryption to restore the decrypted \lstinline|byte[]| to the original \lstinline|String|. However, the APIs are not interchangeable\footnote{In contrast, synonyms are usually interchangeable in natural language settings.}. 
%Besides, the dependence path along with the \lstinline|Cipher| decryption operations does not tell which one to suggest. Another dependence path that includes the API method used to covert the original \lstinline|String| to \lstinline|byte[]| before the encryption tells us which API to suggest. Thus, 
We show that capturing multiple dependence paths can help for precise suggestions in such cases.
\par}

%We present new neural network modeling approaches to overcome the aforementioned shortcomings. From the program analysis aspect, we apply interprocedural program slicing backward from the query API method call to gather a program slice of all influencing code. A program slice can be treated as a minimized program that is required for making the recommendation. However, a program slice can still be complicated, because multiple dependencies interact with each other. Therefore, we further simplify a slice as an API dependence graph by connecting the API methods having direct data dependence (e.g, \lstinline|def-use| chain) together. We make the API recommendations based on the multiple dependence paths of method calls extracted from the API dependence graph.
%\sloppy{
To address the above challenges, we present a neural network-based API recommendation technique called Multi-HyLSTM. Our approach achieves high top-1 accuracy, making it better suitable for real-world usage, compared to existing approaches. Our key insight is to build API embeddings guided by program analysis techniques, and to use neural network architectures that are better suited for programming languages. 

Multi-HyLSTM relies on program analysis to extract more complete dependence relations and represent them as dependence-aware embeddings. In this process, we construct API dependence graphs on program slices to specify data dependence paths between 
API methods. The dependence paths are used to train our dependence-aware embedding (i.e., vectorized representation of code elements) representing the API methods and associated constants. 
%\par}
Multi-HyLSTM differs from existing sequential models as it incorporates multiple dependence paths reaching the query place to generate accurate recommendations.
Compared with the state-of-the-art sequential models (e.g., LSTM, BERT), our approach is better at capturing rare API patterns, as well as long-range complex dependencies. 
%}

%in Multi-HyLSTM is to take program analysis guidance in embedding and apply neural networks tailored for programming languages.


% Our ultimate API recommendation solution Multi-HyLSTM achieves high top-1 accuracy. Our unique insight in Multi-HyLSTM is to take program analysis guidance in embedding and apply neural networks tailored for programming languages. 
% %and includes designs of both program analysis and neural networks. 
% %\fixme{This paragraph is about program analysis, but the first line talks about neural network modeling. Should be something like `We design a program analysis technique to capture the dependencies between APIs and data, and their programming contexts.'???} 
% From the program analysis aspect, we extract more complete dependence relations and represent them as dependence-aware embeddings. In this process, 
% %we gather all the influencing dependencies into a program slice via interprocedural backward program slicing. 
% %A program slice can be complicated due to multiple dependencies between APIs and data. Therefore, 
% we construct API dependence graphs on slices to specify data dependence paths between 
% %direct data dependence (e.g., \lstinline|def-use| chain)  
% API methods. The dependence paths are used to train our dependence-aware embedding (i.e., vectorized representation of code elements). 
% %and make prediction for the next API in the path. %We train the dependence-aware embedding for the API methods and associated constants and make the API recommendations based on the multiple dependence paths extracted from the graph.
% \par}
%We also make several significant improvements in neural network design.
%First of all, we train the dependence-aware embedding to represent the API elements including the API methods and associated constants. The embedding is produced by combining the skip-gram model~\cite{mikolov2013efficient} with the data dependence paths extracted by program analysis. Then, we explore the top-1 accuracy of the state-of-the-art sequence model long short-term memory (LSTM) network, and bidirectional encoder representations from transformers (BERT)~\cite{devlin2018bert} on recommending the Java cryptographic API methods. 
%We first apply the skip-gram model on the dependence paths to get the dependence-aware embeddings for each API elements (i.e., the API methods and associated constants). Embedding represents each API method or constant as a low-dimensional vector reflecting their dependence relationships. Moreover, we present an enhanced model called HyLSTM to improve the accuracy by capturing low-frequency patterns in dependence paths. In addition, based on our high accuracy of recognizing dependence paths, we design a multi-path neural network architecture that takes multiple dependence paths reaching the query place to produce the accurate recommendation. The multiple dependence paths of API method calls are taken by our HyLSTM model separately and aggregated later to decide the optimal recommendation. We design that architecture specifically for the code structure where one location is decided by multiple dependencies.
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/example_illustrate_for_challenges.png}
    \caption{\small{Examples illustrating the two programming specific challenges and how we fix them.}}
    \vspace{-1em}
    \label{fig:example_frequency}
\end{figure*}
% Multi-HyLSTM differs from the sequential model as it incorporates multiple dependence paths reaching the query place to generate accurate recommendations.
% %The goal is to amortize the impact of wrong predictions suggested by one or more paths. Under this new architecture, we present an enhanced model called HyLSTM to take each single dependence path. 
% Compared with the state-of-the-art sequential models (e.g., LSTM, BERT), our model is also better at capturing rare API patterns. %Accurately capturing the less frequent API patterns in the single dependence paths improves the accuracy significantly. %Besides, a single suggestion may depend on multiple dependence paths. 
%To aid the neural network models, we also convert the dependence paths to embeddings for API methods and their associated constants where embeddings express each API method or constant as a low-dimensional vector with their dependence relationships. 

The API recommendation work closest to us is SLANG~\cite{raychev2014code}, which also relies on the combination of program analysis and deep learning approach. Compared to SLANG, we extract more complete dependence information. More importantly, we develop new machine learning techniques to recognize rare and complex API patterns. Our evaluation shows that Multi-HyLSTM outperforms SLANG in capturing more comprehensive dependencies and making more accurate top-1 recommendations.

%The code completion work closest to us is SLANG~\cite{raychev2014code}, which also relies on the combination of program analysis and deep learning approach. In contrast, we extract more complete dependence information. More importantly, we present multiple machine learning innovations for recognizing rare and complex API patterns.    

We extensively evaluate our approach with Java cryptographic code extracted from Android apps. We choose Java cryptographic code because the associated APIs are notoriously complex and error-prone~\cite{chen2019reliable,afrose2019cryptoapi}. The evaluation includes two parts. First, we compare the top-1 accuracy of our Multi-HyLSTM with the state-of-the-art SLANG~\cite{raychev2014code} and a commercial IDE plugin Codota~\cite{codota}. 
%%Multi-HyLSTM shows significant advantages on the top-1 accuracy, 13.97\% higher than SLANG and 24.08\% higher than Codota, respectively. 
Second, we conduct extensive comparative analysis to measure the effectiveness of each design choice via a new metric, \textit{in-set accuracy} (See Section~\ref{sec:eval_design}). This new metric measures accuracy of top-1 recommendations that fall in a plausible next API method set. We collect the next API method set for every input sequence from our dataset by considering the multiple available choices.  
%that evaluates how many top-1 recommendations are reasonable (See Section~\ref{sec:eval_design}). 
%Multi-HyLSTM achieves the best \textit{in-set accuracy} of 98.99\%.  

% We substantially evaluate our solution with Java cryptographic code extracted from Android apps. We choose Java cryptographic code because the associated APIs are notoriously complex and error-prone~\cite{chen2019reliable,afrose2019cryptoapi}. The evaluation includes two parts. First, we compare the top-1 accuracy of our Multi-HyLSTM with the state-of-the-art SLANG~\cite{raychev2014code} and a commercial IDE plugin Codota~\cite{codota}. Multi-HyLSTM shows significant advantages on the top-1 accuracy, 13.97\% higher than SLANG and 24.08\% higher than Codota, respectively. Second, 
% %in our Multi-HyLSTM, including program analysis and dependence-aware embedding, HyLSTM model and multi-path architecture. 
% we conduct extensive comparative analysis to measure the effectiveness of each design choice via a new metric \textit{in-set accuracy} that evaluates how many top-1 recommendations are reasonable (See Section~\ref{sec:eval_design}). Multi-HyLSTM achieves the best \textit{in-set accuracy} of 98.99\%.  

%This paper makes the following contributions:
%\item \fixme{In my opinion, the following paragraph should be the first contribution, feel free to modify/remove if not.} We design a program analysis technique to capture the dependencies between APIs and data, and their programming contexts. We present an enhanced model called HyLSTM that can capture less frequent API usage patterns along with the most frequent patterns in their dependence paths. We also design a multi-path neural network architecture to incorporate multiple dependence paths reaching the query place and generate accurate recommendations.
%\item  We evaluate the top-1 recommendation accuracy of our proposed approach on 36,029 Java cryptographic API method invocations extracted from Android apps and compare it with the state-of-the-art API completion tool SLANG~\cite{raychev2014code}. Our approach achieves the top-1 accuracy of 91.41\%, much higher than SLANG's 77.44\%. We conduct a manual analysis on 245 randomly selected test cases to compare our approach with a state-of-the-art commercial IDE plugin Codota~\cite{codota}. Our method generates substantially more accurate API recommendation with the top-1 accuracy at 88.98\% compared with Codota that achieves the top-1 accuracy at 64.90\%. 

Our key findings are summarized as follows.
\begin{itemize}
\item We evaluate the top-1 recommendation accuracy of Multi-HyLSTM on over 36K Java cryptographic API method invocations. Multi-HyLSTM achieves a top-1 accuracy of 91.41\%, a 14\% improvement over SLANG's~\cite{raychev2014code} accuracy of 77.44\%. We also conduct a manual analysis to compare Multi-HyLSTM with a state-of-the-art commercial IDE plugin Codota~\cite{codota} using 245 randomly selected test cases. Our method generates substantially more accurate API recommendations with a top-1 accuracy of 88.98\%, a 24\% improvement over Codota's top-1 accuracy of 64.90\%.
%%Multi-HyLSTM shows significant advantages on the top-1 accuracy, 13.97\% higher than SLANG and 24.08\% higher than Codota, respectively. 
  
 
%  \item We evaluate the top-1 recommendation accuracy of our Multi-HyLSTM on 36,029 Java cryptographic API method invocations. Our Multi-HyLSTM achieves the top-1 accuracy of 91.41\%, much higher than SLANG's~\cite{raychev2014code} accuracy of 77.44\%. We also conduct a manual analysis to compare Multi-HyLSTM with a state-of-the-art commercial IDE plugin Codota~\cite{codota} using 245 randomly selected test cases. Our method generates substantially more accurate API recommendations with the top-1 accuracy of 88.98\% compared to Codota's top-1 accuracy of 64.90\%.

\item  Multi-HyLSTM achieves the best \textit{in-set accuracy} at 98.99\%. 
 It shows substantial accuracy improvement over BERT (from 55.73\% to 83.02\%) on previously unseen cases.

 
%  \item  Multi-HyLSTM achieves the best \textit{in-set accuracy} at 98.99\%. 
%  %By applying this multi-path architecture on our HyLSTM and BERT models, the \textit{in-set accuracy} increases 3.2\% and 3.29\%, respectively, from their single-path counterparts. In addition, 
%  The multi-path architecture shows substantial accuracy improvements over the single-path HyLSTM and BERT (from 74.44\% to 83.02\%, from 55.73\% to 76.07\%, respectively) on previously unseen cases.

\item  We obtain the program-analysis guided embedding \textit{slice2vec} and \textit{dep2vec} for representing API methods and constants. %We compare it with the one-hot encoding, and two intermediate embeddings, \textit{byte2vec} and \textit{slice2vec}, that are obtained by applying our program analysis guidance partially (i.e., without our interprocedural slicing or API dependence construction). 
Compared with the one-hot encoding on byte code that does not have program-analysis guidance, \textit{slice2vec} and \textit{dep2vec} both show substantial improvements on the \textit{in-set accuracy} by 28\%, 36\%, respectively.


%\item  We obtain the dependence-aware embedding \textit{dep2vec} for representing these API methods and constants. We compare it with the one-hot encoding, and two intermediate embeddings, \textit{byte2vec} and \textit{slice2vec}, that are obtained by applying our program analysis guidance partially (i.e., without our interprocedural slicing or API dependence construction). 
%Compared with the one-hot encoding on byte code, \textit{slice2vec} and \textit{dep2vec} both show substantial improvements on the \textit{in-set accuracy} by 28\%, 36\%, respectively.

%while the \textit{byte2vec} makes no significant difference. %The dependence paths are better choice to model API usage compared with slices and bytecode sequences.  reaching the accuracy of 92.35\% compared with the baseline 55.80\%.

\item 
%\fixme{this contribution is unclear and distracting.} 
 HyLSTM, the important building block of Multi-HyLSTM, achieves an excellent \textit{in-set accuracy} (93.00\%) on single dependence paths. HyLSTM shows 13.73\% higher \textit{in-set accuracy} on previously unknown cases over a regular LSTM model.     


    

\end{itemize}




We also publish a large-scale Java cryptographic code dataset \footnote{ \url{https://github.com/Anya92929/DL-crypto-api-auto-recommendation}} for evaluating embedding and suggestion model designs. It includes the code corpora of bytecode, slices, and data dependence paths. 


==> Comprehensive Comparisons of Code Embedding Methodologies for Java Cryptographic Applicatons/Sections/2-technical_challenges_and_overview.tex <==












%\begin{lstlisting}[frame=TB,language=Java,caption={A code example of calculating message digest. The API and constant sequences are highly entangled. Analysis on  only one method is insufficient to inference the secure usage. },captionpos=b,label={lst:code_example}]
%private MessageDigest getDigest(String algo) {
%    try { return MessageDigest.getInstance(algo);
%    } catch (NoSuchAlgorithmException e) {
%        throw new RuntimeException(e.getMessage());}}
%public byte[] calculate_digest(int mode, String key) {
%    byte[] bytes = key.getBytes();
%    MessageDigest md = null;
%    if mode==0:
%        md = getDigest("MD5");//Insecure
%    else:
%        md = getDigest("SHA-256")//Secure
%    return md.digest(bytes);
%}
%\end{lstlisting}


%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{images/multi-path_challenge_illustrate.png}
%    \caption{An example of the functionally similar APIs that require multi-path to distinguish. (a) shows two API dependence graphs. According to dependence paths $P_1$ and $P_2$, g1 and g2 have similar programming context. Only when considering $P_3$, they can be distinguished.}.
%    \label{fig:example_multi_path}
%\end{figure}






\begin{figure*}
    \centering
    \includegraphics[width=.8\linewidth]{images/components.png}
    \vspace{-1.5em}
    \caption{\small{Main components of our API recommendation solution Multi-HyLSTM and the overview of our comprehensive comparative setting}}
    \label{fig:overview}
    \vspace{-1.5em}
\end{figure*}


\section{Technical Challenges and Research Questions}
\label{sec:challenges}




% Ya, I commented below out, as we've talked about it in the intro, so I think the readers should get it by now.
%\smallskip
%\noindent
%{\em How to solve the program-specific entanglement in the API and constant embedding and suggestion? }
%Programs are not processed following the sequential order. Program-specific entanglement, caused by method invocation, flexible statement order, etc, widely exists in various program  representations (e.g. source code, byte code, etc). Figure~\ref{fig:code_entanglement} shows the API and constant sequences extracted from the same piece of code with different program analysis preprocessing. The entangled order in Fig.~\ref{fig:seq_byte} and Fig.~\ref{fig:seq_slice} introduces fake relationship in their embeddings. The location-based code coverage may miss critical program influences from other program locations. Our approach leverages program slicing to break the location boundary and deliver the dependence-based coverage for suggestion. 


%

We discuss two programming language-specific challenges that hinder accurate API method recommendations. 
We use the term \textit{API pattern} to refer to the subsequence of API methods that frequently appear in the data-dependence paths. 
We call two API patterns sharing a common subsequence as the \textit{variant of each other}.



\smallskip
\noindent
%{\em Design challenge: how to recognize low-frequency long API sequences that have high frequency suffixes?}
{\em Design challenge 1: how to recognize the low-frequency variant of a high-frequency API pattern?}

Some API patterns are used more frequently than their variants, making it difficult to recognize their low-frequency variants. The end result is that the model only predicts the frequent API pattern.
An example is shown in Figure~\ref{fig:example_frequency}(a). The subsequence ($b, c, d_2$) is a high-frequency pattern in our extracted data-dependence paths. However, when the prefix is a special one (e.g., $a_1$), the last API method should be $d_1$, instead of $d_2$. This phenomenon is common in real codebases. 
%Should we convince readers by code example?
We find that native LSTM models are unable to identify the low-frequency variant (i.e., $a_1, b, c, d_1$) because of the frequency imbalance. 
%different from the common pattern (i.e., $b,c,d_2$),  


% Some API patterns are used much more frequently than their variants, causing it difficult to recognize these low-frequency variants. The end result is that the model only predicts the frequent API pattern.
% An example is shown in Figure~\ref{fig:example_frequency}(a). The subsequence ($b, c, d_2$) is a high-frequency pattern in our extracted data-dependence paths. However, when the prefix is a special one (e.g., $a_1$), the last API method should be $d_1$, instead of $d_2$. This phenomenon is common in the codebase. 
% %Should we convince readers by code example?
% We found that native LSTM models are unable to identify the variant (i.e., $a_1, b, c, d_1$) different from the common pattern (i.e., $b,c,d_2$),  because of the frequency imbalance. 

To address this issue, we present a new sequential model HyLSTM by modifying the LSTM loss function (Section~\ref{sec:hylstm}). Our idea is to give a strong signal to the model about the different patterns. We amplify the importance of the last token (e.g., node $d_1$ and $d_2$) in the entire sequence to calculate the sequence loss. Our experiments verify that this new amplified loss function in HyLSTM makes the model better at identifying low-frequency variants. We use HyLSTM as an important building blocks of our Multi-HyLSTM.
%gives the model better capability of identifying low-frequency variants. 


%We address this issue by modifying the loss function of the LSTM sequence model training as shown in Section~\ref{sec:hylstm}. Intuitively, we give a strong signal to the model about the different patterns. We amplify the importance of the last token (e.g., node $d_1$ and $d_2$) in the entire sequence to calculate the sequence loss. Our experiments verify that this new amplified loss function gives the model better capability of identifying low-frequency variants. 

%We found native LSTM models are unable to differentiate multiple long sequences that share a common subsequence. 
%
% Daphne commented below sentence out, need to rephrase to point out the problem exists in a regular LSTM, not in our invented model
%Our experiments also confirm that all of these different sequences sharing a common subsequence end up with the same label, causing wrong code predictions for these low-frequency invariant patterns. 
%Two similar input sequences, say (a, c, d, e, f) and (b, c, d, e, f), with different target g and h, respectively, would generate similar hidden states $h(a, c, d, e, f)$ and $h(b, c, d, e, f)$, which is undesirable. The influences from their first token is minimized because the majority sequences having this common suffix (c, d, e, f) following different prefixes (not only a) suggest the label g. Their similar hidden states are very likely to make identical predictions, making the infrequent one to be misled by a more frequent pattern. 
% It is challenging to tell different faraway prefixes apart in  sequences sharing common subsequences. 
%
%The last APIs are different and decided by the prefix (i.e. when \lstinline|GCM| is used). However, the model cannot recognize it because the majority cases follow the Figure~\ref{fig:global_influence_example}a that almost ignore what the prefix is. 
%




\smallskip
\noindent
{\em Design challenge 2: how to differentiate different APIs that share similar functionality?} 

In Java APIs, even though slightly different APIs may share the same functionality, they cannot be used interchangeably. The prediction model needs to know when to use which API. Existing work does not address this challenge. In Figure~\ref{fig:example_frequency} (c), the API methods $g_1$ and $g_2$ work in a similar programming context. According to the dependence paths $P_1$ and $P_2$, there is no indicator showing which one should be used. To distinguish them, a critical path $P_3$ should be captured. We find that many functionally-similar API methods follow this property.   
%For example, \lstinline|Cipher.init(int,Key,AlgorithmParameters)| and \lstinline|Cipher.init(int,Key)| both work for cipher initialization and share several identical dependence paths, making them indistinguishable. 
For example, \lstinline|new String(byte[])| and \lstinline|Base64.Encoder.encodeToString(byte[])| both work for encoding \lstinline|byte| arrays into a \lstinline|String| after the identical \lstinline|Cipher| decryption operations. The shared dependence paths make them indistinguishable. 
Our approach is to incorporate all the dependence paths from their arguments to increase the coverage for the critical dependencies (e.g., previous decoding behaviors for this example). Our recommendation is therefore made by leveraging multiple dependence paths. 


% In Java APIs, even though slightly different APIs may share the same functionality, they cannot be used interchangeably. The prediction model needs to know when to use which API. Existing work does not address this challenge.
% As shown in Figure~\ref{fig:example_frequency} (c), the API methods $g_1$ and $g_2$ work in similar programming context. According to the dependence paths $P_1$ and $P_2$, there is no indicator showing which one should be used. To distinguish them, a critical path $P_3$ should be captured. We found that many functionally-similar API methods follow this property.   
% For example, \lstinline|Cipher.init(int,Key,AlgorithmParameters)| and \lstinline|Cipher.init(int,Key)| both work for cipher initialization and share several identical dependence paths, making them indistinguishable. Our approach is to incorporate all the dependence paths from their arguments to increase the coverage for the critical dependencies. Our recommendation is made under the influences of multi-paths. 




%This imbalance issue is program-specific and has not been reported in natural languages literature.  The long-range influences is ignored by the model because it is suggested as less important in majority sequences following the Fig.~\ref{fig:global_influence_example} pattern.  To make accurate suggestion, the model need to be sensitive enough for the long-range influences making differences. 

%how to be sensitive enough for less-frequent but important long-range influences?}
%For code suggestion, subsequences that repeatedly appear can easily be identified as patterns by a machine learning model (e.g., LSTM). We observe that some general short patterns much more frequent than their longer variants in the extracted code sequences. 

%The API \lstinline|Cipher.getInstance(String)| is used to create a cipher object. Then this cipher object is required to be initialized with a key through \lstinline|Cipher.init(int,Key)|. Finally, the byte array to be encrypted can be fed into the cipher through API \lstinline|Cipher.doFinal(byte[])| to finalize the encryption. 

%\smallskip
%\noindent
%{\em Evaluation challenge: How to validate the success of a model design?}
Our work also systematically compares various design choices for neural-network-based API recommendations. We make substantial efforts to confirm the effectiveness of a model design through comparative experiments. Our research questions are: 
%multiple ways, including {\em i)} direct comparison of code prediction accuracy, {\em ii)} comparison against baseline models, {\em iii)} incremental model designs for comparison purposes, and {\em iv)} manual case studies on failed or successful cases. Our evaluation methodologies and our datasets are useful beyond the specific code suggestion problem.


\begin{itemize}
    \item RQ1: Does our approach outperform the state-of-the-arts in terms of the top-1 recommendation?
    \item RQ2: How  much  do  program-analysis  insights  improve  API recommendation?
    \item RQ3: How  to  recognize  low  frequency  long  API  sequences?
    \item RQ4: How  to  accurately  differentiate  different APIs that share the same functionality?
\end{itemize}


%To differentiate them, the minor differences are required to be highlighted. We leverage the differences of their arguments to differentiate them. We collect the dependence paths for all of their arguments and design a model architecture to deal with these sequences in parallel. Every single dependence paths are pretrained separately through the sequential language model. Their sequence embeddings are incorporated with identical importance in the task training phase.  Therefore, the code suggestion is made by taking multiple argument dependencies into consideration.  





==> Comprehensive Comparisons of Code Embedding Methodologies for Java Cryptographic Applicatons/Sections/3-our_approaches.tex <==



\section{Design of Multi-HyLSTM }

We describe the key design choices of our Multi-HyLSTM. We start by introducing our dependence-aware embedding guided by static program analysis. The static analysis draws the data dependence paths that are required to make accurate API recommendations. Based on the extracted dependence paths, embedding maps thousands of cryptography-related API methods and constants to the dependence-aware vectors of a low dimension (e.g., 300). We then describe the new neural network model designed for high-precision API recommendation, including the multi-path architecture and a low-frequency long-range-enhanced model called HyLSTM.
%including {\em multi-path architecture} and the HyLSTM model that enhances the low-frequency long API patterns.
%
%In this section, we present the three critical components of our neural-network-based code suggestion solution, {\em program-analysis-guided embedding}, {\em long-range-enhanced sequence learning}, and {\em multi-path code suggestion}. 
%
%For  program-analysis-guided embedding, we describe multiple static analysis  pre-processing strategies to reduce noises in raw sequences and bring the dependence context for embedding. 
%For long-range-enhanced sequence learning, we introduce a target amplification strategy for LSTM to emphasize the infrequent but important long-range influences.  
%For multi-path code suggestion, we aggregate program context from multiple dependence paths to better differentiate function-similar APIs in suggestion. 
The main components of our approach and the overview of our comparative analysis are illustrated in Figure~\ref{fig:overview}.

%{\bf Ya, i'd like to visualize the api to vector mapping to provide a more visual explanation for readers about embeeding. so for fig 3, the "code embedding" box, i wonder whether can replace the current drawing with something illustrating embedding, like mapping apis into vector? 

%you can increase the width of that box if needed, as we still got a bit width. what do you think?}

% Ya, below is confusing to me, I commented out. 
%We give a multi-dependence based code suggestion solution based on the program-analysis guided embeddings in the first part and global influence aware sequence embedding in the second part.

\subsection{Program-analysis-guided Embedding}\label{sec:embedding}



We specialize lightweight static data-flow analysis techniques to preprocess code sequences before embedding them. The embedding of API methods and constants act as the input vectors of our neural network model. By applying the static analysis, our approach aims to effectively leverage programming language insights to capture dependence relations in embedding vectors.
%Unlike pure data-driven solutions (e.g., one-hot encoding\footnote{A straightforward vector representation of tokens assuming tokens are independent of each other.}), our approaches aim to effectively leverage language insights to capture the required program context for embedding. 

%As shown in Figure~\ref{fig:overview}, we leverage inter-procedural backward slicing to extract program slices from Android bytecode. Then, we build the API dependence graphs on each program slices. The purpose of the program analysis is to break the location boundary of code representation and gather useful program context for the neural networks to learn. 

\noindent
%\smallskip
{\sc Inter-procedural backward slicing.} 
   We start the inter-procedural backward slicing from the invocation statement of a cryptography API. The slicing criteria are its arguments. All the code statements influencing the API invocation are organized together to form a program slice. Self-defined method calls are replaced by their code body statements. By eliminating the non-influencing code statements and breaking the method boundary, the program slices guarantee the required information program-wide as well as keeping the code size minimum. It also partially disentangles the API and constant sequences as shown in Fig.~\ref{fig:overview}.
   
   

\noindent
%\smallskip
{\sc API dependence graph construction.}
On the program slice, we build the API dependence graph by adding data dependence edges on its control flow graph. Then, we simplify this graph as a high-level API dependence graph (see Fig.~\ref{fig:overview}), in which each node is an API or a constant, by merging the non-API nodes. It significantly reduces the size of a graph and connects two data-dependent APIs. %We extract embedding context from the dependence paths of these graphs.  




%We applied the skip-gram model for code embedding.  Beside the regular context based labeling strategy, we present a novel dependence pair . 

%\noindent
%\smallskip
%{\sc High-level Context Extraction.} An API or constant is usually surrounded by many SyntaxTokens~\cite{rahman2019natural} and variable names that have few impact on the API usage. Therefore, to make the model concentrate on API usage, we extract its high-level context, nearby APIs and constants, as the labels in skip-gram to train the embedding vector.   

%\noindent
%\smallskip
%{\sc Dependence Pair Extraction.} Many security-concerned tokens (e.g. \lstinline|MD5| and \lstinline|SHA-256|) are interchangeable in code, making their embedding indistinguishable according to the extracted context. To differentiate them as well as not compromising their semantic similarity, we presented a new labeling strategy to use their dependence pairs to train their embedding, referred to as DP labeling. It uses the embedded token itself and its immediate successor as labels for skip-gram~\cite{mikolov2013distributed}. 
 
 
 %Figure~\ref{fig:byte_slice_dep} illustrate the API and constant context extracted from byte code, program slices and API dependence graph, respectively. For the purpose of comparison, we train embeddings from byte code, program slices, and API dependence graph, respectively, to reveal the effectiveness of the program-analysis-guided strategies. 



 
We apply skip-gram embedding model~\cite{mikolov2013distributed} on the byte code, slices, and dependence paths extracted from the API dependence graphs, respectively, to produce three types of Java cryptography embeddings, \textit{byte2vec}, \textit{slice2vec}, and \textit{dep2vec}.  %We scientifically compare these design choices based on their performance in code suggestion tasks. The code embedding part in 
Figure~\ref{fig:overview} gives simple examples.


\begin{itemize}
    \item \textit{byte2vec} is the baseline embedding version that applies \textit{word2vec} \cite{mikolov2013efficient,mikolov2013distributed} directly on the byte code corpus.
    \item  \textit{slice2vec} is the embedding with the inter-procedural backward slicing as the pre-processing method.
    \item  \textit{dep2vec} applies two pre-processing techniques, inter-procedural backward slicing, and API dependence graph construction, to guide the embedding training. 
    %\item  \textit{sDep2vec} is the embedding that involves the most program-specific customizations. \textit{sDep2vec} uses the dependence pair labeling strategy. Its embedding training is performed on data flows of API dependency graphs, which are built on inter-procedural backward slicing, as in \textit{dep2vec}.  
\end{itemize}



%{\bf Ya, should we explain "dependence pair labeling strategy" a bit more? like at least 1-2 sentences? otherwise reviewers will complain, as we never explain it elsewhere either, right? 

%another option is to completely remove sdep2vec, which is better?}
\begin{figure}[b]
\vspace{-1em}
    \centering
    \includegraphics[width=\linewidth]{images/multi_path_selection.png}
    \caption{\small{Multiple Paths Selection for API Recommendation. We use the information associated with the nodes and edges to select paths. The goal is to maximize the coverage for different nearby branches with minimal paths.}}
    \label{fig:path_selection}
    \vspace{-1em}
\end{figure}
\subsection{Multi-path API Recommendation}\label{multi_hyLSTM}

%{\bf Ya, I've done switching the 2 subsections and other places in sections 1 and 2, as well. To do for you: in this section, please slightly revise the writeup to present multi-path independent of HyLSTM. Avoid mentioning HyLSTM here. This technique is not strictly relying on HyLSTM right? So that'd make multi-path look more general and useful.

%Then, at the end of this section 3, say a few words about integrating them two in your experiments. }

We design a new multi-path architecture and apply it on top of the sequential language models to address the challenge caused by functionally-similar-yet-non-interchangeable APIs. Instead of making API recommendations based on a single sequence, our new model incorporates multiple related data dependence paths. This design allows the model to have a more comprehensive view of the data flows, thus producing more accurate predictions.  The training of multi-path API recommendation model includes three operations: {\sc multi-path selection}, {\sc path-embedding training}, and {\sc multi-path aggregation}.
The multi-path architecture leverages the efficiency and performance success achieved by sequence models that are more efficient than the graph-based neural networks that suffer the scalability issue.
%{\bf Ya, how does this multi-path differ from the graph-based approaches in related work, please explain briefly in the paragraph above. thanks.}

\smallskip
\noindent
{\sc Multi-path Selection.} 
The number of paths in an API dependence graph sometimes explodes. To minimize the computational cost, we apply our multi-path selection algorithm to limit the number of paths (to five in our experiments) that are input to neural networks. Intuitively, our goal is to \textbf{maximize} the coverage of different nearby data and control flow branches with a \textbf{minimal} number of paths. Specifically, we traverse the paths backward from the target node to the beginning node. At each branch, we apply the breadth-first search to select the edges that deliver different flow-in variables or belong to different control flow branches. 

As illustrated in
Figure~\ref{fig:path_selection},
%illustrates an API dependence graph including many paths beyond our path budget.  
there are flow-out and flow-in variables associated with each edge and control dependence information associated with each node. 
%In the API dependence graph, we record the flow-out and flow-in variables for each data dependence edge. 
%This design enables us to recognize the edges delivering different variables to a destination. For each node, we record its control dependent node to differentiate the predecessors belonging to different control flow branches. 
%Our goal is to maximize the coverage of the flow-in variables and different control flow branches. 
%We first check all the incoming edges of our target node about the flow-in variables delivered by them. We select one predecessor for each flow-in variable as the more-important predecessors. 
For node 11, there are two edges from node 8 and node 10, respectively, delivering identical flow-in variables $\$r1$. One can select either one of them. In this example, node 8 and node 13 that deliver different variables are selected to continue the path traversal.  
%That ensures the selected paths to be diverse and cover different data flow branches.
If there are two predecessors that deliver identical flow-in variables but belong to different control flow branches, we also add both of them in this step. We continue this breadth-first backward traversal process until the path budget has been used up. After that, each selected branch will be completed as a complete path by the depth-first search to an arbitrary beginning node.  This greedy breadth-first approach guarantees the local optimal choice at every branch. Since the nearby dependencies are more important than the faraway ones, our backward traversal prioritizes the coverage of the nearby dependencies. 
%The diversity of the dependence paths helps us to generate more accurate recommendation.

%There are many function-similar APIs that only differ in parameter lists. The path for the distinct flow-in variable is a strong signal to differentiate them.  For the edges delivering identical flow-in variable with a selected path, we check the control dependence of their predecessors. If they belong to different control flow branches, we trace for this edge and add the path that only differs from the existing one in the control-flow branch part.  The two paths provide
%complementary information to distinguish the function-similar APIs that are used in different phases. %Both the \lstinline|Cipher.doFinal()| and \lstinline|Cipher.update(byte[])|  are encrypting operations. However, the former is used as the final one while the latter is used in early phase. 


\smallskip
\noindent
{\sc Path Embedding Training.} To better understanding each path, we generate the sequence embedding, the vectors for an entire sequence, by pretraining the language model with all the separate dependence paths extracted from the API dependence graphs. The language model takes these sequences as input and is trained at every step to predict the next token. Every token of this sequence is represented as the \textit{dep2vec} embedding we trained for each cryptographic API and constants in Section~\ref{sec:embedding}. We use the hidden state vector after the last timestep as the embedding for the input sequence. This vector describes the probability distribution of the next API usage given this path $P(t_n|(t_0,t_1,\dots,t_{n-1}))$. This sequence model is fine-tuned later under the multi-path architecture. 
%We apply this architecture trained BERT model to generate the sequence embedding for comparison purposes. We use the masked language model task to train BERT and produce the sequence embedding.



\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/multi_path_suggestion.png}
    \caption{\small{Multi-path Code Suggestion based on aggregating the Path Embedding}}
    \label{fig:multi_path_suggestion}
    \vspace{-1.5em}
\end{figure}

\smallskip
\noindent
{\sc Multi-path Aggregation.} Based on the selected multiple dependence paths, we predict the next API by aggregating their sequence embedding vectors. As shown in Figure~\ref{fig:multi_path_suggestion}, the pretrained sequence model is set as the initial state.  Each of them produces path embedding that suggests the next token $t_n$ according to $P(t_n|(t_0,t_1,\dots,t_{n-1}))$. We add an average pooling layer to aggregate these path embeddings into one vector that represents $ave(P(t_n|path\ i))$. The prediction is generated from that aggregated vector with the softmax classifier. Under the multi-path architecture, the sequence model is jointly updated with the following layers towards the task-specific distribution.  The multi-path architecture successfully highlights the minor difference in the process of code suggestion.   Candidate tokens having similar probabilities in some paths can be accurately differentiated based on their probability difference from an extra path. We applied this multi-path architecture on the sequence model BERT and HyLSTM, an advanced LSTM model proposed by us, in Section~\ref{sec:multi-path} to demonstrate the effectiveness of our approach.




\subsection{Low-frequency Long-range-enhanced Learning}\label{sec:hylstm}

%Although our disentangled sequences and dependence-aware embedding make substantial breakthrough in learning code sequences, it is still difficult for regular LSTM sequence model to captured the low-frequency long-range influences and make accurate code suggestions on it. 
%
\begin{figure}
    \centering
    \includegraphics[width=.66\linewidth]{images/hylstm.png}
    \caption{\small{Target amplification in HyLSTM with our new hybrid loss function.}}
    \label{fig:hylstm}
    \vspace{-1.5em}
\end{figure}

%Considering the fact that the majority code sequences rely on nearby dependence context while a few of them cares about far-away context, the accurate suggestion requires the model to be more sensitive for those impactful far-away context. 
Under the multi-path architecture, each dependence path is handled by a sequence model presented by us, referred to as HyLSTM. HyLSTM is designed for addressing the challenge posed by the low-frequency API method sequences with a high-frequency suffix, as we demonstrate in Figure~\ref{fig:example_frequency}. Intuitively, we solve this issue by forcing the model to assign larger weights to beginning tokens (e.g., $a_1$ in Figure~\ref{fig:example_frequency}) when needed, making beginning tokens more useful for predicting the API (e.g., $d_1$). 




HyLSTM differs from the regular LSTM sequence model in its architecture and loss function. 
We show our HyLSTM in Figure~\ref{fig:hylstm}. It includes two parallel output layers $FCL_1$ and $FCL_2$ after the LSTM cells while regular LSTM based sequence learning only has the $FCL_2$.  The output of $FCL_1$ is the target (i.e., the recommended API method) of the given dependence path while the $FCL_2$ outputs every intermediate token of the given path.  %The detail is shown as follows.


%{\bf Ya, i trust you will add key sentences in this section to improve readability for SE researchers, as we discussed. mind the semantic gap. thanks.}

As regular LSTM, the hidden states $h_i$ at every timestep are taken by the fully connected layer  $\mbox{\em FCL}_2$ to output the next token in the forward propagation. 
\begin{align}
\begin{bmatrix}
s_1\\ 
s_2\\ 
\dots\\ 
s_{n}
\end{bmatrix}= \mbox{\em softmax}(\begin{bmatrix}
h_0\\ 
h_1\\ 
\dots\\ 
h_{n-1}
\end{bmatrix} W_2 +\begin{bmatrix}
B_2\\ 
B_2\\ 
\dots\\ 
B_2
\end{bmatrix})
\end{align}
where $W_2$ and $B_2$ are the weights and bias for $\mbox{\em FCL}_2$.

In HyLSTM, we add an extra parallel fully connected layers $\mbox{\em FCL}_1$ to accept the hidden layer at the last timestep $h_{n-1}$. $\mbox{\em FCL}_1$ outputs the prediction $o_{n}$ by:
\begin{align}
 o_{n} = \mbox{\em softmax}( h_{n-1} W_1 + B_1)
 \end{align}
 where $W_1$ is a weight matrix and $B_1$ is the bias vector for $\mbox{\em FCL}_1$.
 
 We define a hybrid loss combining the losses from the two fully connected layers. The goal of this design is to guarantee that the hidden states $h_{n-1}$ are distinguishable to reproduce the different targets via $FCL_1$, as well as maintain the similarity at the intermediate steps via $FCL_2$.
 
%$s_i$ 
%The $o_n$ is responsible for the next token while $s_i$ encodes the intermediate representation at each timesteps. 
%The last hidden state $h_{n-1}$ is guided simultaneously by the target and entire sequence. 

The new hybrid loss $l_h$ is defined as:
\begin{align}
l_h = \alpha  L(o_n,x_n)+ (1-\alpha) \sum_{i=1}^{n}\frac{L(s_i,x_i)}{n}
\end{align}
where $L(\cdot)$ is the cross entropy loss between the output and label. We set  $\alpha$ to be 0.5 in our experiments.

%In conventional models, hidden states are supervised at every timestep by the corresponding successor. As a result, two similar input sequences, say (a, c, d, e, f) and (b, c, d, e, f), with different target g and h, respectively, would generate similar hidden states $h(a, c, d, e)$ and $h(b, c, d, e)$, which is undesirable. In other words, conventional LSTM models minimize the difference in the first token after supervision by identical label series, (c, d, e, f). Accepting one more identical input token f, their similar hidden states $h(a, c, d, e, f)$ and $h(b, c, d, e, f)$ are very likely to make identical predictions, making the low frequent one to be misled by a high frequent pattern. This frequency imbalance cannot be simply addressed by sampling techniques because the full sequences displaying a high frequent pattern may still be different. 

When low-frequency sequences were initially predicted wrong due to its misleading high-frequency suffix, HyLSTM produces a larger loss than regular LSTM to correct it and treat the beginning tokens more seriously.
%Two similar sequences resulting in different targets are emphasized by $\mbox{\em FCL}_1$.  Simultaneously, $\mbox{\em FCL}_2$ guarantees their similarity in the intermediate hidden states to keep the inference capability. In this way, the influences of longer patterns having different targets $x_n$ are maintained in $h_{n-1}$ even though they are infrequent.  
Besides evaluating HyLSTM against regular LSTM models, we also compare it with BERT in Section~\ref{sec:experimental_results}.


 
 
 %Intuitively, 
%our hybrid loss function effectively assigns larger weights to beginning tokens (e.g., $a_1$ in Figure~\ref{fig:example_frequency}) than standard LSTM, making beginning tokens more useful for predicting the API (e.g., $d_2$). Larger weight helps counter the influence of high-frequency suffixes. 
%when low-frequency sequences were initially predicted wrong due to its misleading high-frequency suffix. In response, HyLSTM produces larger loss than standard LSTM to correct it and treat beginning tokens more seriously. As a result, our hybrid loss function effectively assigns larger weights to beginning tokens (e.g., $a_1$ in Figure~\ref{fig:example_frequency}) than standard LSTM, making beginning tokens more useful for predicting the API (e.g., $d_2$). Larger weight helps counter the influence of high-frequency suffixes.
 

\smallskip
\noindent
{\em Integration of multi-path architecture and HyLSTM.}
We apply our multi-path architecture on top of HyLSTM to make API recommendations with high accuracy, which produces our Multi-HyLSTM model. 
%The HyLSTM is used to better inference the next token considering a single dependence path. The multi-path aggregation makes accurate suggestions by incorporating the influences from the multiple paths.
%{\bf Ya, please rearrange the text and say a few sentences here. }

%{\bf Ya, in the last sentence above, "close probability" --> similar probabilities? 

%differentiate --> differentiated?

%probability distinction --> probability difference?
%}







 
 







==> Comprehensive Comparisons of Code Embedding Methodologies for Java Cryptographic Applicatons/Sections/4-dataset_and_experimental_setup.tex <==
\section{Datasets and Experimental Setups}\label{sec:dataset_setup}

%{\bf Ya, this dataset description needs to be shortened.}

%\subsection{Datasets}

We collect two datasets of 36,641 and 12,335 apps from the Google Play store, respectively. 
%to evaluate the proposed approaches.  
To build a diverse dataset, we select the most popular apps from different categories in the app store and filter them to guarantee that these  apps use Java cryptographic APIs. 
%Out of the 16K apps, 12,335 apps  implement cryptography functionalities. 
%We filter the irrelevant code and only keep the classes that use the JCA and JCE packages.
The former dataset is used to train and evaluate the API method and constant embedding. The latter is used for downstream tasks training and evaluation.  

%We collect 16,048 Android Applications from the google market to form the dataset. 
%We choose Android Apps because Cryptography functional code is more likely to appear in high-level services that require data transmission, authentication, etc. 
%To diverse the cryptography functional code, 

%Our dataset covers different application categories including communication, business, and finance.  We select the most popular apps in each category to download.  Not all of the applications implement cryptography functionalities. We filter the irrelevant code and only keep the classes that use the JCA and JCE packages.

%6,291 apps belong to the finance category. 4,581 of them are communication applications. The other 5,176 apps are in the business category. 



To build embeddings, the following three types of code corpora are extracted during pre-processing: {\em i) byte code}, {\em ii) slices}, and {\em iii) dependence paths}. Their size is shown in Table~\ref{tab:stats_corpora}. The tokens include the APIs or constants we aim to embed. APIs include the standard APIs from Java and Android platforms, as well as some third party APIs that cannot be inlined because they are recursive or phantom (whose bodies are inaccessible during the analysis). We filter APIs to embed those that appear more than 5 times. Besides, we manually collect 104 reserved string constants used as the arguments of cryptographic APIs. The 104 constants along with the constants that appear more than 100 times in the slice corpus are used for embedding. Finally, we have 4,543 tokens (3,739 APIs and 804 constants) in the embedding vocabulary. 


\begin{table}[t]
\centering
\caption{\small{Statistics of embedding corpora size}}
\label{tab:stats_corpora}

\begin{tabular}{baba}
\Xhline{2\arrayrulewidth}
\rowcolor{Gray}
\textbf{Corpora} & \textbf{Byte code} & \textbf{Slices} &  \begin{tabular}[c]{@{}c@{}}\textbf{Dependence}\\ \textbf{paths}\end{tabular}  \\ \hline
\textbf{\# of tokens} & 28,887,852 & 12,341,912 & 38,817,046 \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\vspace{-0.5em}
\end{table}

\begin{table}[ht]
\centering
\caption{\small{Composition of the embedded APIs}}
\label{tab:composition_apis}

\begin{tabular}{lla}

\Xhline{2\arrayrulewidth}
\rowcolor{Gray}
\multicolumn{2}{c}{\textbf{Source}} & \multicolumn{1}{l}{\textbf{\# of embedded APIs}} \\ \hline
\hline
\multicolumn{1}{l|}{\multirow{5}{*}{Java platform}} & \multicolumn{1}{l|}{java.security} & 510 \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{javax.crypto} & 166 \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{java.io} & 138 \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{java.lang} & 259 \\
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{others} & 374 \\ \hline
\multicolumn{2}{l|}{Android platform} & 486 \\ \hline
\multicolumn{2}{l|}{Third parties} & 1827 \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\vspace{-1em}
\end{table}
%There are three embedding code corpora extracted from different code representations after our pre-processing.  They are {\em i) byte code}, {\em ii) slices}, and {\em iii) dependence paths}. The size of the three corpora is shown in Table~\ref{tab:stats_corpora}. The tokens of them are the APIs or constants we aim to embed.


%There are three embedding code corpora extracted from different code representations after our pre-processing.  They are {\em i) byte code}, {\em ii) slices}, and {\em iii) dependence paths}. The size of the three corpora is shown in Table~\ref{tab:stats_corpora}. The tokens of them are the APIs or constants we aim to embed.
%There are 7,189 APIs and 10,497 constants in the embedding vocabulary.   
%APIs include the standard APIs from Java and Android platform, as well as some third parties' methods that cannot be inlined because they are recursive or phantom (whose bodies are inaccessible during the analysis). We filter APIs to embed those that appear more than 5 times. For constants, we manually define a list of 104 reserved string constants used as the arguments of cryptographic APIs. The list of 104 constants along with the constants that appear more than 100 times in the slice corpus are used for embedding.
%We filter the constants with a higher threshold than APIs because many constants are user-defined like file names. They usually do not repeat across programs. 
%Finally, we have 4,543 tokens (3,739 APIs and 804 constants) in the embedding vocabulary. 





%\smallskip
%\noindent
%{\em Slices vs. dependence paths vs. byte code}

Table~\ref{tab:naturalness_of_data} shows the number of sequences extracted from different code corpora.
Compared with byte code, slices and dependence paths have more sequences, but less \textbf{unique} sequences.
%The naturalness hypothesis \cite{hindle2012naturalness,ray2016naturalness,hindle2016naturalness} points out that programming (source) code is highly repetitive, which is why it is possible to learn with probability models. 
%Producing a model to recognize 262,448 sequences (byte code) is more difficult than training one to handle 23,128 traces (dependence paths). This analysis, as well as our experimental results, 
This suggests that learning under the guidance of program-analysis is more desirable than learning on byte code.
%which confirms that learning under the guidance of program-analysis is more desirable than learning on byte code. 
To guarantee fairness, we subsample the extremely frequent dependence paths as \cite{mikolov2013distributed} without losing the unique paths. The total number of paths after subsampling is 566,279, which has a close total/unique ratio with slices. 
%proportional to the slices according to their unique sequences. \bimal{what do you mean proportional? rephrase?}

\begin{table}[b]
\centering
\vspace{-1em}
\caption{\small{Number of sequences parsed from different representations}}
\vspace{-1em}
\begin{tabular}{|b|a|b|a|}
\hline \hline
\rowcolor{Gray}
\textbf{}       & \textbf{\begin{tabular}[c]{@{}c@{}}Byte\\ code\end{tabular}} & \textbf{Slices} & \textbf{\begin{tabular}[c]{@{}c@{}}Dependence\\  paths\end{tabular}} \\ \hline  \hline
\textbf{Total}  & 707,775                                                         & 926,781          & 4,655,763                                                              \\ \hline
\textbf{Unique} & 262,448                                                         & 54,173           & 23,128                                                                \\ \hline  \hline
\end{tabular}
\vspace{-1.5em}
\label{tab:naturalness_of_data}
\end{table}
%\subsection{Experimental Setup}
 
 

\smallskip
\noindent
{\em Experimental setup of program analysis pre-processing}.
%
To get slices, we develop a crypto slicer that is inter-procedural, context- and flow-sensitive. We use the open-source Java program analysis framework Soot~\cite{vallee2010soot} for pre-processing. Soot takes the Android byte code as input and transforms it into an intermediate representation (IR) Jimple. The program analysis is performed on Jimple IR. Our slicer using Soot's BackwardFlowAnalysis framework works with Soot 2.5.0, Java 8, and Android SDK 26.1.1. 


\smallskip
\noindent
{\em Experimental setup for embedding}. 
%
We use the same hyperparameters decided by our preliminary experiments for all the embedding training. The embedding vector length is 300. The sliding window size for neighbors is 5. We also applied the subsampling and negative sampling to randomly select 100 false labels to update in each batch. We train embeddings with the mini-batch size of 1024. The embedding terminates after 10 epochs. %The experiments about the impact of these hyperparameters are in Table~\ref{tab:hyper_param_embedding1} and ~\ref{tab:hyper_param_embedding2} in the Appendix. 
Our embedding model is implemented using Tensorflow 1.15. Training runs on the Microsoft AzureML GPU clusters, which supports  distributed training with multiple workers. We use a cluster with 8 worker nodes. The VM size for each node is the (default) standard NC6. 
 

\smallskip
\noindent
{\em Experimental setup for API recommendation tasks}.
%
%We extract the API and constant sequences from byte code, program slices, and API dependence graphs, respectively. In byte code, we collect sequences at method-level. We discard the methods that only include one token (API or constant) in our vocabulary. In API dependence graphs, we extract the dependence paths to form the sequence dataset. 
We filter the vulnerable code using CryptoGuard~\cite{rahaman2019cryptoguard}, which is a cryptography API misuse detection tool based on program analysis. Only secure code is kept to avoid data poisoning~\cite{schuster2020you}. 
%We evaluate how well the embedding vectors are by applying them to the sequential code suggestion task. To avoid the bias from the downstream task itself, we defined two code suggestion tasks with different model architectures and difficulty levels. 
We limit the maximum number of input steps to 10 (truncate sequences longer than 10). 
%Within each batch, the sequences are padded the same length. We also apply masking to eliminate the impact of padding when updating the model. 
We use batch size of 1,024, and learning rate of 0.001. We select the highest accuracy achieved within 10 epochs because we observe that the accuracy increase is negligible after that. 
%We applied LSTM-based models and BERT-based models with different design choices in our code suggestion tasks for comparison purposes. 
% {\sc Code token suggestion} is to predict the next token (i.e., API or constant), given an API and constant sequence. 
 %For the sequences ($x_0, x_1, \dots, x_n$), we use ($x_0, x_1, \dots, x_{n-1}$) and ($x_1, x_2, \dots, x_n$) as the input and outputs of the model in Figure~\ref{fig:hylstm}. 
We use the stacked LSTM architecture with vanilla LSTM cells for the LSTM-based models. For the BERT model, we use 12 attention headers and the hidden size is 256. 



%{\em In-set accuracy.}  A code sequence may have multiple reasonable next tokens according to our dataset. We collect the next token set for every input sequence from our dataset and calculate the in-set accuracy according to whether the prediction falls in the next token set.

%According to different evaluation purposes, we calculate the accuracies with minor changes. When evaluating the impacts of pre-processing and embedding strategies in the code token/sequence suggestion tasks, we measure the accuracy under a simplified scenario, i.e. making sure one input sequence only has one following tokens in training. When evaluating our model designs for the code suggestion, we measure a \textit{in-set accuracy} to better understand the model suggesting capability. The \textit{in-set accuracy} measures whether the prediction falls in a reasonable next token set we collected according to the ground truth of our dataset.%In the tasks evaluating the embedding quality, we use the accuracy of  

%However, a code sequence may have multiple choices for the next $k$ tokens. According to different evaluation purposes, we calculate the accuracies with minor changes. When evaluating the impacts of pre-processing and embedding strategies in the code token/sequence suggestion tasks, we measure the accuracy under a simplified scenario, i.e. making sure one input sequence only has one following tokens in training. When evaluating our model designs for the code suggestion, we measure a \textit{in-set accuracy} to better understand the model suggesting capability. The \textit{in-set accuracy} measures whether the prediction falls in a reasonable next token set we collected according to the ground truth of our dataset.%In the tasks evaluating the embedding quality, we use the accuracy of  
%We collect the next token set for every input sequence from our dataset and calculate the in-set accuracy according to whether the prediction falls in the next token set.
    
    
%\noindent
%{\sloppy
%{\sc Code sequence suggestion} is to produce a sequence of following APIs or constants, given an incomplete API and constant sequence.  We use the LSTM sequence to sequence model for this task.  
% The original sequences are separated into two non-overlapping parts, ($x_0, x_1, \dots, x_{[n/2]}$) and ($x_{[n/2]+1}, x_{[n/2]+2},\dots, x_{n} $) as the input and target output of the model, respectively.
%The sequence-to-sequence LSTM model is composed of an auto-encoder and an auto-decoder. We use two vanilla LSTM cells for the auto-encoder and auto-decoder. We also limit the number of maximum extended steps of the auto-encoder and auto-decoder to 10, respectively (truncate the original sequence longer than 20). For the training process, we use batch size 1,024, and the default learning rate of 0.001. The training is terminated after 30 epochs as we observe that the accuracy increase is negligible after that.
% \par}

%{\bf Ya, the tasks description can be shortened too.}






==> Comprehensive Comparisons of Code Embedding Methodologies for Java Cryptographic Applicatons/Sections/5-experimental_results.tex <==




  \begin{table*}[!b]
\caption{\small{The top-1 recommendation accuracy of Codota plugin and our Multi-HyLSTM on 245 randomly selected Java Cryptographic API invocation test cases. Codota gives recommendation based on the previous code and the return value while we only assumes that the previous code is known. We show our default accuracy without the return value and the improved version when the return value type is considered.} }\label{tab:codota}
\begin{small}
\begin{tabular}{|b|a|b|a|b|a|}
\hline
\hline
\rowcolor{Gray}
                                                        &  &  &  & \multicolumn{2}{c|}{\textbf{Multi-HyLSTM (Our approach) Accuracy}}  \\  \cline{5-6}  
\rowcolor{Gray} \multirow{-2}{*}{\textbf{App Category}} &  \multirow{-2}{*}{\textbf{\# of Test Cases}}                                    &            \multirow{-2}{*}{\textbf{\# of Apps}}                          &                     \multirow{-2}{*}{\textbf{Codota Accuracy}}                    & w/o return value         & with return value        \\ \hline \hline
Business                               & 66                                         & 3                                    & 66.67\%                                   & 89.39\%                  &    98.49\%                      \\ \hline
Finance                                & 99                                         & 3                                    & 65.66\%                                   & 90.91\%                  & 97.98\%                         \\ \hline
Communication                          & 80                                         & 3                                    & 62.5\%                                    & 86.25\%                  &   97.59\%                       \\ \hline
\textbf{Total}                                  & \textbf{245}                               & \textbf{9}                           & \textbf{64.9\%}                           & \textbf{88.98\%}         & \textbf{97.96\%}                \\ \hline \hline
\end{tabular}
\end{small}
\vspace{-1em}
\end{table*}


\section{Experimental Evaluation}\label{sec:experimental_results}

Our evaluation includes two parts. First, we evaluated the effectiveness of our Multi-HyLSTM with top-1 recommendation accuracy. We compare our accuracy results with the state-of-the-art tool SLANG~\cite{raychev2014code} and a commercial IDE plugin Codota~\cite{codota}. Second, we conducted extensive comparative experiments to analyze the accuracy capability of each design choice shown in Table~\ref{tab:comparative_setting}. The objective of this part is to study how effective these design choices are in terms of improving accuracy compared with some intermediate solutions and answer a couple of research questions. 

\noindent
\textbf{Evaluation Metrics.}
There are two metrics in our evaluation. We use the top-1 accuracy to evaluate our approach Multi-HyLSTM and two state-of-the-art tools SLANG and Codota on recommending the next API method. When evaluating the design choices (e.g., embedding vs. one-hot encoding, HyLSTM vs. LSTM) through the intermediate solutions, we introduce a new metric, referred to as \textit{in-set accuracy}.  
We use this new metric because we noticed that in the intermediate solutions, a code sequence (e.g., a dependence path) may have multiple correct choices for the next API method call. Therefore, we define \textit{in-set accuracy} as the accuracy of top-1 recommendations that fall in a reasonable next API method set. We collect the next API method set for every input sequence from our dataset by considering the multiple available choices. Compared with the top-$k$ accuracy, \textit{in-set accuracy} guarantees that the top-1 recommendation is a reasonable choice. 

\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{images/multi_hylstm_slang_acc.pdf}
    \vspace{-1em}
    \caption{\small{The top-1 accuracy of SLANG and our approach on recommending Java cryptographic API method calls from Android Applications }}~\label{fig:slang}
   \vspace{-1.5em} 
\end{figure}


\subsection{Top-1 Recommendation Accuracy}\label{sec:recom_eval}

%[Mention it in Dataset section] To evaluate the accuracy capability of recommending complex APIs, we 

% Should we mention SALAD and explain why we did not compare with it?
\sloppy{
We perform experiments to answer our first research question (\textit{RQ1: Does our approach outperform the state-of-the-arts in terms of the top-1 recommendation?}). 
 We select two state-of-the-art API recommendation tools, SLANG~\cite{raychev2014code} and Codota~\cite{codota}, for comparison. SLANG completes the next API method based on program analysis and statistical language models. Codota is a commercial AI code completion plugin, which is adopted by the mainstream IDEs including IntelliJ, Eclipse, Android Studio, VS Code, etc. \par}



\noindent
\textbf{Comparison with SLANG}
 We locate 36,029 Java cryptographic API method callsites from the bytecode of the 16,048 Android Applications. By applying the required static analysis, our method and SLANG extract corresponding program context for these cryptographic API method callsites. We randomly select 1/5 of the callsites as the test cases and train SLANG and our model with the other 4/5 cases.    
%SLANG differs from our approach in two aspects. First, SLANG extracts multiple partial object histories while we extracts multiple data dependence paths as the input context. Second, 
SLANG combines the $n$-gram and RNN models to generate the probability of the next API method call. 
%In \cite{raychev2014code}, Raychev et al. choose 3-gram and RNN model with units 40. 
We try different $n$ for the $n$-gram model and different hidden layer sizes for the RNN model of SLANG and our Multi-HyLSTM model.     

Figure~\ref{fig:slang} shows the top-1 accuracy of SLANG and our approach under different configurations. We choose the hidden layer size of SLANG and our approach from 128, 256, and 512. With each hidden layer size setting, we also adjust SLANG with 3-gram, 4-gram, 5-gram model~\footnote{Raychev et al choose 3-gram and hidden layer size 40 for RNN in \cite{raychev2014code}}. Our approach shows significant advantages over SLANG under all settings. The highest top-1 accuracy of SLANG is 77.44\%, achieved with RNN-256. The $n$-gram model shows no impact on the top-1 accuracy. Our models achieves the best accuracy at 91.41\% under Multi-HyLSTM with hidden layer size 512. 







\noindent
\textbf{Comparison with Codota}
Given an incomplete code statement with an object with a \verb|dot| in an IDE, Codota displays a ranked list of the recommended API methods associated with the object. We randomly selected 245 cryptographic API method invocations from 9 Android applications as the test cases. We decompiled the 9 apps into source code and load them into IntelliJ IDE with Codota. Then, we manually triggered Codota recommendation by removing the method name after the \verb|dot|. The accuracy results are shown in Table~\ref{tab:codota}.  Our approach has a significant improvement on the top-1 accuracy compared with Codota. The top-1 accuracy of the 245 cases is improved from 64.90\% to 88.98\%. 

Codota takes not only the previous code but also the return value into consideration to give compatible recommendations. This is different from our approach which only relies on the previous code. 
%To support the more difficult scenario that the developers do not know the return value and the object holder of the method call, our approach gives recommendation only with the previous code. 
For fair comparison, we add an extra manual evaluation on all these 245 test cases. We manual checked the return value type and use it to filter our recommendation candidates output from the neural network model.  Our top-1 accuracy (last column in Table~\ref{tab:codota}) rises to 97.96\% if the return type is known. 









\subsection{Evaluation on Design Choices}\label{sec:eval_design}


\begin{table*}[htpb]
\vspace{-1em}
\caption{\small{The comparison settings of our comprehensive comparative analysis. Group 1 controls on our program analysis and embedding techniques. Group 2 focuses on the effectiveness of our low-frequency long-range enhancing technique. Group 3 reveals the improvement from the multi-path architecture. }}\label{tab:comparative_setting}
\vspace{-1em}
\begin{scriptsize}
\begin{tabular}{b|ababab|ab|abab}
\hline \hline
\rowcolor{Gray}  &\multicolumn{6}{c|}{Group 1 (RQ2)} & \multicolumn{2}{c|}{Group 2 (RQ3)} & \multicolumn{4}{c}{Group 3 (RQ4)}
\\ \cline{2-13}
    \rowcolor{Gray}              Our design choices                                       & \begin{tabular}[c]{@{}c@{}}1-hot on\\ bytecode\end{tabular} & byte2vec & \begin{tabular}[c]{@{}c@{}}1-hot on\\ slices\end{tabular} & slice2vec & \begin{tabular}[c]{@{}c@{}}1-hot on\\ dependence \\ paths\end{tabular} & dep2vec & HyLSTM & \begin{tabular}[c]{@{}c@{}}LSTM \\ (token-level or \\ sequence-level loss)\end{tabular} & \begin{tabular}[c]{@{}c@{}}HyLSTM\\ (path embedding)\end{tabular} & BERT & Multi-HyLSTM & Multi-BERT \\ \hline \hline
\begin{tabular}[c]{@{}c@{}}Interprocedural \\ program slicing\end{tabular}   & \emptycirc                                                           & \emptycirc        & \fullcirc                                                 & \fullcirc     & \fullcirc                                                                 & \fullcirc    & \fullcirc   & \fullcirc                                                             & \fullcirc                                        & \fullcirc                        & \fullcirc       & \fullcirc     \\ \hline
\begin{tabular}[c]{@{}c@{}}API dependence \\ graph construction\end{tabular} & \emptycirc                                                   & \emptycirc        & \emptycirc                                                   & \emptycirc     & \fullcirc                                                               & \fullcirc  & \fullcirc   &\fullcirc                                                           & \fullcirc                                           & \fullcirc                       &\fullcirc       & \fullcirc      \\ \hline
\begin{tabular}[c]{@{}c@{}}Token-level\\ embedding\end{tabular}                                                                    & \emptycirc                                                         & \fullcirc    &\emptycirc                                                   & \fullcirc      & \emptycirc                                                               & \fullcirc   & \fullcirc     & \fullcirc                                                               & \fullcirc        & \fullcirc                                                           & \fullcirc          & \fullcirc        \\ \hline
\begin{tabular}[c]{@{}c@{}}Low frequency long\\ range enhancing\end{tabular} & \emptycirc                                                        & \emptycirc     & \emptycirc                                                 & \emptycirc       & \emptycirc                                                               & \emptycirc   & \fullcirc & \emptycirc    & \fullcirc                                                             & \emptycirc                                                              & \fullcirc          & \emptycirc     \\ \hline
\begin{tabular}[c]{@{}c@{}}Path-level\\ embedding\end{tabular}                                                     & \emptycirc                                                   & \emptycirc     & \emptycirc                                                   & \emptycirc     & \emptycirc                                                               & \emptycirc  & \emptycirc   & \emptycirc                                                            & \fullcirc                                        & \fullcirc                         & \fullcirc        & \fullcirc     
\\ \hline
\begin{tabular}[c]{@{}c@{}}Multi-path\\ architecture\end{tabular}                                                     & \emptycirc                                                   & \emptycirc     & \emptycirc                                                   & \emptycirc     & \emptycirc                                                               & \emptycirc  & \emptycirc   & \emptycirc                                                            & \emptycirc              & \emptycirc                                                    & \fullcirc        & \fullcirc       \\ \hline \hline
\end{tabular}
\end{scriptsize}

\end{table*}
We evaluate the effectiveness of our design choices  by comprehensive comparative experiments between the intermediate solutions. The intermediate solutions apply different combinations of our design choices. We demonstrate our comparative setting in Table~\ref{tab:comparative_setting}. %Our experiments aim to study the accuracy capability of 1) different forms of program analysis context, 2) the sequence model choices, and 3) the multi-path architecture designed for code structure and answer the research questions in Section~\ref{sec:challenges}. %Specifically, we focus on the following research questions.



\subsubsection{RQ2: How  much  do  program-analysis  insights  improve  API recommendation?}
We answer this research question with the comparative experiments in the group 1 of Table~\ref{tab:comparative_setting}. 
%three forms of program context, 1) the byte code sequences, 2) the program slices, and 3) the dependence paths, combined with the embedding technique. 

We compare these settings with two types of API recommendation tasks, i.e., {\em next API recommendation} and {\em next API sequence recommendation}. The former aims to predict one API method to be used in the next line while the latter produces a sequence of API methods to be invoked sequentially. 
%We extract the API methods and constants sequences from the three forms of context. They work with identical neural network settings to output API recommendations.  
We use the regular LSTM based sequence model for the next API method task. In the next API sequence recommendation task, we use the LSTM based seq2seq (encoder-decoder) model to accept the first half API element sequence and predict the last half API elements. %We truncate the sequences to limit the maximum input length as 10.  %These are native LSTM based models without our long-range-enhanced design and multi-path architecture. 

\begin{table}[b]
\vspace{-1.5em}
\centering
\caption{\small{Accuracy of next API Recommendation.}}
\begin{scriptsize}
\vspace{-1em}
\begin{tabular}{|c|a|b|a|b|a|b|}
\hline \hline
\rowcolor{Gray}
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}LSTM\\ Units\end{tabular}}} & \multicolumn{2}{c|}{\textbf{Byte Code}} & \multicolumn{2}{c|}{\textbf{Slices}} & \multicolumn{2}{c|}{\textbf{Dependence Paths}} \\ \cline{2-7} 
                                                                               & 1-hot               & byte2vec           & 1-hot         & slice2vec         & 1-hot       & dep2vec          \\ \hline \hline
\textbf{64}                                                                    & 49.78\%            & 48.31\%            & 66.39\%         & 78.91\%          & 86.00\%      & 86.33\%        \\ \hline
\textbf{128}                                                                   & 53.01\%            & 53.52\%            & 68.51\%         & 80.57\%          & 84.81\%      & 87.75\%         \\ \hline
\textbf{256}                                                                   & 54.91\%            & 54.59\%            & 70.35\%         & 82.26\%          & 84.57\%      & 91.07\%           \\ \hline
\textbf{512}                                                                   & \textbf{55.80\%}            &    \textbf{55.96\%}                 &  \textbf{71.78}\% &           \textbf{83.35}\%        &  \textbf{86.34} \%      & \textbf{92.04\%}         \\ \hline \hline
\end{tabular}
\label{tab:task1}
\end{scriptsize}
\vspace{-1em}
\end{table}









\noindent
{\em Comparison setting.} There are two groups of comparison. First, we compare the in-set accuracy between the models trained on the bytecode sequences, program slices, and dependence paths to reveal the benefit of the program analysis. Second, we add the API elements embedding on the corresponding sequence corpora and compare them with the one-hot encoding counterparts. Altogether, we have three intermediate baselines, one for each of the bytecode sequences, slices, and dependence paths. This group aims to show the improvement of the embedding technique combined with program analysis. %In the dependence paths corpus, an $n$ token sequence may be followed by many different subsequences ($n+1\mbox{\em -th}$ to $n+k\mbox{\em -th}$ tokens). We only use the most frequent one to train and test the model. This setting is only applied for experiments aiming to answer RQ1.  


%{\bf Ya, below should be Tables -- plural form. check similar situations, e.g., paths 1 and 2, not path 1 and 2. thanks.}
Tables~\ref{tab:task1} and ~\ref{tab:task2} evaluate the program-analysis guided embedding quality by the next API recommendation task and the next API sequence recommendation tasks, respectively. 
%Tables~\ref{tab:task1} and ~\ref{tab:task2} show the embedding quality evaluation through the code token suggestion task and the code sequence suggestion tasks, respectively. 
Compared with the basic one-hot on byte code (no program-specific designs are applied), the models trained with \textit{slice2vec} and \textit{dep2vec} achieve much higher accuracy in both tasks. The highest accuracies (92\% and 89\%) of both tasks are achieved by \textit{dep2vec}, which are 36\% and 46\% higher than their baseline settings, respectively. 

{\sloppy 
\noindent
\textit{Comparison between different program analysis techniques.}  Program analysis preprocessing techniques show significant benefits. For the next API recommendation task, the accuracy under one-hot encoding setting is improved from 56\% (one-hot on byte code) to 72\% (one-hot on slices) by inter-procedural slicing, and further to 86\% (one-hot on dependence paths) by the API dependence graph construction.  Under the embedding setting, the accuracy with \textit{slice2vec} is 27\% higher than \textit{byte2vec}.  The accuracy with \textit{dep2vec} is 92\%, 9\% higher than \textit{slice2vec}. The results of the next API sequence recommendation are also consistent with the conclusion. Comparison among the three one-hot settings shows that inter-procedural slicing improves the task accuracy by 20.5\%\footnote{64.10\% - 43.61\%=20.5\%}; API dependence graph construction improves the task accuracy by 18.8\%\footnote{82.94\% - 64.10\%=18.8\%}. \par}

\noindent
{\em Comparison between embedding and one-hot encoding.}  Results are shown in Table~\ref{tab:task1} and ~\ref{tab:task2}. There are significant improvements by applying embeddings on slices and dependence paths. In the next API recommendation task, \textit{slice2vec} improves the accuracy by 11\% from its one-hot baseline. \textit{dep2vec} improves the accuracy by 6\% from its one-hot baseline. These improvements suggest that \textit{slice2vec} and \textit{dep2vec} capture helpful information in vectors. In contrast, there is no significant improvement from applying embedding to the (unprocessed) byte code corpus. This conclusion is also observed in the next API sequence recommendation task. \textit{slice2vec} and \textit{dep2vec} improve the accuracy from their baselines by around 21\% and 6\%, respectively.  In contrast, \textit{byte2vec} does not show any significant improvement from its one-hot baseline.
 %
%For the code token suggestion, there is no significant difference between the results of \textit{dep2vec} (91.07\%) and \textit{sDep2vec} (92.35\%).  Recall that \textit{sDep2vec} uses transitive labeling, whereas \textit{dep2vec} uses conventional neighbor-based labeling. Our results suggest transitive labeling is not critical for the code generation tasks. 

The impact of the LSTM units is as expected.  Longer LSTM units have higher accuracy.  Furthermore,  the accuracy increases more rapidly from LSTM-64 to LSTM-128 compared with LSTM-256 to LSTM-512.  It is likely because once the model has enough capacity, the differences caused by embedding are smaller. 
 


 \begin{table}[t]
 \centering
 \caption{\small{Accuracy of the Next API Sequence Recommendation. We use the LSTM with hidden layer size 256 for this task.}}

\begin{tabular}{|b|a|b|a|b|a|}
\hline \hline
\rowcolor{Gray}
\multicolumn{2}{|c|}{\textbf{Byte Code}} & \multicolumn{2}{c|}{\textbf{Slices}} & \multicolumn{2}{c|}{\textbf{Dependence Paths}} \\ \hline 
1-hot           & byte2vec       & 1-hot        & slice2vec    & 1-hot    & dep2vec      \\ \hline \hline
43.61\%        & 44.63\%        & 64.10\%     & 85.02\%     & 82.94\%    & 89.23\%      \\ \hline \hline
\end{tabular}
\vspace{-1.5em}
\label{tab:task2}
\end{table}

%\smallskip
%\noindent
%{\sc Experimental Results of Code Sequence Suggestion.}
%Based on the results of the code token suggestion, we only apply the LSTM with the units 256 for this task.  The accuracy results in code sequence suggestion are mostly consistent with those of code token suggestion. The best result (89\% accuracy) comes from the models trained with \textit{dep2vec}. It is a substantial improvement from the baseline model's 44\% accuracy. The model trained with \textit{slice2vec} also achieves a high accuracy of 85\%.  

 




\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/case_study1.pdf}
\caption{\small{Case Study 1. (a) {\em slice2vec} and its one-hot slice baseline both incorrectly predict the test case. (b) {\em dep2vec} based on the dependency graph shown make the correct prediction.}}
\label{fig:case_study1}
\vspace{-1.5em}
\end{figure}

\smallskip
\noindent
{\sloppy
{\em Case Study 1.}  This case study is on the effectiveness of the API dependence graph construction. Figure~\ref{fig:case_study1}(a) shows a slice-based test case that is mispredicted by both {\em slice2vec} and its one-hot baseline. For digest calculation, it is common for \lstinline |MessageDigest.update(.)| to be followed by \lstinline |MessageDigest.digest(.)|, appearing 6,697 times in training. However, Figure~\ref{fig:case_study1}(a) shows a reverse order, which is caused by the \verb1if1-\verb1else1 branch shown in Figure~\ref{fig:case_study1}(b). When \lstinline |MessageDigest.update(.)| appears in an \verb1if1 branch, there is no guarantee which branch would appear first in slices. This reverse order is less frequent, appearing 1,720 times in training. Thanks to the API dependence graph construction, this confusion is eliminated, which predicts this case correctly. 

%From dependency perspective, it is quite common that \lstinline |MessageDigest.getInstance(.)| is followed by either \lstinline |MessageDigest.update(.)| or \lstinline|MessageDigest.digest(.)|, appearing 28072 times and 26435 times, respectively. When they both appear, \lstinline |MessageDigest.update(.)| is always before \lstinline |MessageDigest.digest(.)|, because the latter finalizes \lstinline |digest| calculation. This ordering appears 6697 times. 

 

\par}












\smallskip
\noindent
{\sloppy
{\em Case Study 2.} This case study is on the ability to recognize new previously unseen test cases. The slices in Figure~\ref{fig:case_study2}(a) and Figure~\ref{fig:case_study2}(b) slightly differ in the arguments of the first API. {\em slice2vec} makes the correct predictions in both cases, while its one-hot baseline fails in Figure~\ref{fig:case_study2}(a).
\lstinline |MessageDigest.getInstance(String)| appears much more frequent than \lstinline |MessageDigest.getInstance(String,Provider)| in our dataset. Specifically,  the former API appears 207,321 times, out of which 61,047 times are followed by the expected next token \lstinline |MessageDigest.digest(.)|. In contrast, the latter API -- where one-hot fails -- only appears 178 times, none of which is followed by \lstinline |MessageDigest.digest()|. 
In {\em slice2vec}, the cosine similarity between \lstinline |MessageDigest.getInstance(String,Provider)| and \lstinline |MessageDigest.getInstance(String)| is 0.68.~\footnote{For one-hot vectors, this similarity is 0.} This similarity, as the result of {\em slice2vec} embedding, substantially improves the model's ability to make inferences and recognize similar-yet-unseen cases. 
\par}

\begin{figure}[t]
    \centering

\includegraphics[width=\linewidth]{images/case_study2.pdf}

\caption{\small{Case Study 2. (a) A test case that is correctly predicted by {\em slice2vec}, but incorrectly by one-hot encoding. (b) A test case similar to (a), but both {\em slice2vec} and one-hot give the correct prediction.}}
\label{fig:case_study2}
\vspace{-1.5em}
\end{figure}

%\begin{figure}
%\centering

%\includegraphics[width=\linewidth]{images/case_study3.pdf}

%\caption{Case Study 3, (a) A slice-based test case that is correctly predicted by one-hot encoding, but incorrectly by {\em slice2vec} in task 1 (code token generation). (b) Two code snippets that suggested by the one-hot encoding and {\em slice2vec} predictions, respectively.}
%\label{fig:case_study3}
%\end{figure}

%\smallskip
%\noindent
%{\sloppy
%{\bf Case Study 3.} For task 1, we investigate the reasons behind cases where the one-hot baseline performs better than {\em slice2vec}.
%Figure~\ref{fig:case_study3}(a) shows a two-token sequence from code snippet 1 in Figure~\ref{fig:case_study3}(b).  {\em slice2vec}'s prediction is \lstinline |"AES"|, which does not match the ground truth but is still acceptable. In comparison, the one-hot slice baseline makes the correct prediction.  {\em slice2vec}'s answer (shown in code snippet 2) -- although acceptable -- appears less frequently (twice in training) than the expected answer does (18 times). This frequency difference likely contributes to the observed prediction outcomes. As expected, the one-hot model, specifically trained for this particular task (i.e., task-specific), recognizes high-frequency cases well. 

%This case study suggests an interesting future problem. How to better tailor general-purpose pre-trained code embeddings, like {\em slice2vec}, to specific tasks to help recognize task-specific patterns? One approach is to parameterize the task training to fine-tune general-purpose embeddings further for the task, similar to what is done in~\cite{labutov2013re}.  \par}


%\smallskip
%\noindent
%\fbox{\begin{minipage}{\linewidth}
%Program slicing and API dependence graph construction significantly improve the code embedding quality and code suggestion performance. The dependence paths extracted from the API dependence graphs are the best choice to learn from. The \textit{dep2vec} and \textit{sDep2vec} that are trained from the dependence paths achieves the best code suggestion accuracy.
%\end{minipage}}
\begin{table}[b]
\centering
\vspace{-1em}
\caption{\small{The accuracy of HyLSTM for the next API recommendation. Acc.(A) refers to the in-set accuracy for all the test cases. Acc.(K) is the in-set accuracy for the known test cases. Acc.(U) is the in-set accuracy for new and unknown test cases.}}
\label{tab:hylstm}
\begin{small}
\vspace{-1em}
\begin{tabular}{|b|a|b|a|}
\hline \hline
\rowcolor{Gray}
                        & \textbf{HyLSTM}   & \begin{tabular}[c]{@{}c@{}}
                         \textbf{LSTM}      \\  (token-level loss)
                     
                        \end{tabular} & \begin{tabular}[c]{@{}c@{}}
                           \textbf{LSTM }   \\ (sequence-level loss)
                              
                        \end{tabular}\\ \hline \hline
Acc.(A)     & \textbf{93.00\%}  & 90.77\%    &  90.62\%     \\ \hline
Acc.(K)     & \textbf{99.86\%}      & 99.81\%     & 96.98\%       \\ \hline
Acc.(U)      & 56.94\%     &   43.21\%  &   \textbf{57.13\%}      \\ \hline \hline
\end{tabular}
\vspace{-1em}
\end{small}

\end{table}
\subsubsection{RQ3: How  to  recognize  low  frequency  long  API  sequences?}
We answer this research question with the comparative analysis within group 2 in Table~\ref{tab:comparative_setting}. 
We compare HyLSTM with two intermediate solutions, the LSTM with token-level loss and the LSTM with sequence-level loss, for the next API recommendation task.  The token-level loss is calculated based on the output at the last timestep while sequence-level combines the loss at every timestep of the sequence.
% Instead of HyLSTM, we use LSTM model with token-level loss and sequence-level loss, respectively. 
Their difference is that HyLSTM applies our low-frequency long-range enhancing technique while the others do not.  For all experiments, we use identical LSTM cells with hidden layer size 256.
%We use the LSTM units 256 and our \textit{dep2vec} for all these experiments aiming to compare the model designs.  
We evaluate the {\it in-set accuracy} and further break it down as the in-set accuracy for known and unknown cases as defined below.
%Besides the {\it in-set accuracy} mentioned in Section~\ref{sec:dataset_setup}, we also break it down as the in-set accuracy for known and unknown cases to better understand the suggestion capability of the models.
% we define the metrics to evaluate code suggestion accuracy.
%We calculate three metrics to gain in-depth insights for the accuracy capabilities of the model in generating code suggestions. 

%\smallskip
%\noindent
%{\em In-set accuracy.}  A code sequence may have multiple reasonable next tokens according to our dataset. We collect the next token set for every input sequence from our dataset and calculate the in-set accuracy according to whether the prediction falls in the next token set.


\smallskip
\noindent
{\em In-set accuracy of known cases.} Accuracy of known cases is the in-set accuracy calculated for the test cases that have appeared in the training.  We expect that the enhanced long-range influences could improve the accuracy of known cases.
%These cases are expected to get the correct prediction if the long-range influences have been captured. Therefore, the improvement of experience accuracy may indicates better capability of identifying these low frequency long-range influences. 

\smallskip
\noindent
{\em In-set accuracy of unknown cases.} We calculate the in-set accuracy for new test cases unseen in the training set to see the inference capability of a model.  
%We combine the accuracy for known and unknown cases to avoid overfitting.\bimal{I think the last sentence can be removed. unsure what it's trying to say.}   



As shown in Table~\ref{tab:hylstm}, HyLSTM outperforms the two intermediate solutions in the in-set accuracy by 1.23\%, and 1.38\%, respectively. The token-level loss and sequence-level loss show a trade-off between their accuracy for known cases and unknown cases. The HySLTM combines their strengths, substantially improving the accuracy for unknown cases by 13.73\%, compared with LSTM with token-level loss. HyLSTM also outperforms both intermediate solutions with the almost perfect accuracy for known cases at 99.86\%, without weakening their strengths. According to our manual case studies, most of the failed known cases are caused by the low-frequency API sequences. Therefore, higher accuracy for known cases without sacrificing the unknown cases gives a strong indication about the enhanced long-range influences. 



\begin{figure}[t]
    \centering
    \includegraphics[width=.99\linewidth]{images/case3.png}
    \caption{\small{Case Study 3, (a) A test case that is predicted incorrectly by regular LSTM and correctly by HyLSTM. (b) A test case that follows the frequent short pattern thus got correct prediction by both regular LSTM and our HyLSTM.}}
    \label{fig:case_study_global}
    \vspace{-1.5em}
\end{figure}

\noindent 
{\em Case Study 3.} This case verifies that our HyLSTM is better at identifying the low-frequency long-range patterns. Figure~\ref{fig:case_study_global} (a) shows a test case that is predicted incorrectly by regular LSTM but fixed by our HyLSTM. The regular LSTM makes the wrong prediction because the model is misled by the more frequent pattern shown in Figure~\ref{fig:case_study_global} (b). Compared with the label \lstinline|PKCS8EncodedKeySpec.<init>(byte[])|, the wrong prediction \lstinline|String.<init>(byte[])| is suggested more frequently according to these short suffixes. %The frequency gap is caused by their semantics. \lstinline|String.<init>(byte[])| converts the decrypted data into \lstinline|String| format for displaying. \lstinline|PKCS8EncodedKeySpec.<init>(byte[])| only serves one special purpose, to reconstruct a private key from an encrypted source.    
HyLSTM successfully differentiates the similar inputs from (a) and (b) with the long-range influences enhancing design. 

%{\bf Ya, if you have time later, can we beautify the tables? see some of our group's papers for examples, like adding additional decorative lines, or changing some rows to bold, etc? thank you.}


\subsubsection{RQ4: How  to  accurately  differentiate  different APIs that share the same functionality?}~\label{sec:multi-path}
We answer this question with the comparison within the group 3 in Table~\ref{tab:comparative_setting}. We compare our model with BERT, our multi-path architecture with their single-path counterparts in the next API recommendation task.
%We compare our Multi-HyLSTM approach that uses path embedding and multi-path aggregation with 4 intermediate solutions: (1) Basic HyLSTM (results in Table~\ref{tab:hylstm}), (2) single-path HyLSTM with path embedding, 
%\bimal{is this single path or multi-path? if single-path, then say single-path.}
 %(3) vanilla BERT, and (4) BERT with multi-path architecture. All of them apply our program analysis and embedding technique. The first two also apply our low-frequency long-range enhancing technique. %We use BERT to compare with our HyLSTM in terms of identifying the low-frequency long-range sequences. 
%\bimal{Check this sentence.}

%Multi\_HyLSTM has two extra designs, path embedding and multi-path aggregation, compared to the basic HyLSTM in Table~\ref{tab:hylstm}. We add an intermediate baseline with an extra path embedding phase in Table~\ref{tab:multi_paths}. 
%The Multi\_HyLSTM has two extra designs, path embedding and multi-path aggregation compared with the basic HyLSTM.  and has one extra design, multi-path aggregation compared with the HyLSTM (with path embedding).  %compare the multi-path architecture on HyLSTM and BERT with their single-path baselines, respectively. In their single-path baselines, HyLSTM and BERT is pretrained on another large dependence sequence dataset to obtain the path embedding. Multi\_HyLSTM and Multi\_BERT starts with the path embedding and fine-tune them under the multi-path architecture.

%that leverages the aggregated path embedding with the HyLSTM in Table~\ref{tab:hylstm} as the basic baseline. We also add an intermediate baseline that train HyLSTM with the path embedding pretrained on another large dependence sequence dataset. Besides, we  Experiments in Table~\ref{tab:multi_paths} can be compared with the HyLSTM in Table~\ref{tab:hylstm} as the basic base line. Compared between the HyLSTM (with sequence embedding) here and the basic HyLSTM, we show the improvement caused by the sequence embedding phase. The comparison between the HyLSTM (with sequence embedding) reveals the effect of incorporating multiple dependence paths in prediction. Comparisons between HyLSTM (with sequence embedding) and BERT, Multi\_HyLSTM embedding and Multi\_BERT give the difference between HyLSTM and BERT in prediction code sequences. 
Table~\ref{tab:multi_paths} presents the in-set accuracy results for Multi-HyLSTM and the single-path counterparts. 
The Multi-HyLSTM achieves the best code in-set accuracy at 98.99\%, showing significant improvement (5.99\%) than the basic HyLSTM (Table~\ref{tab:hylstm}). %Both the multi-path HyLSTM and 
%Table~\ref{tab:multi_paths} shows the code suggestion experiments with our multi-path architecture on top of the HyLSTM and BERT, respectively. The Multi\_HyLSTM achieves the best code in-set accuracy at 98.99\%, showing significant improvement (5.99\%) than the basic HyLSTM in Table~\ref{tab:hylstm}. %Both the multi-path HyLSTM and multi-path BERT outperforms their single path intermediate baselines. the multi-path architecture  shows the best suggestion accuracy (98.99\%) achieved our Multi\_HyLSTM. The It displays the suggestion accuracy improvement made by incorporating multiple sequence embeddings for different dependence paths. Multi\_HyLSTM achieves the best suggestion accuracy at 98.99\%, 5.99\% higher than the basic HyLSTM shown in Table~\ref{fig:hylstm}. 
\begin{table}[b]
\centering
\vspace{-1.5em}
\caption{\small{Comparison between multi-dependence suggestion and sequential suggestion. A, K, and U stand for in-set accuracy for all cases, known cases, and unknown cases, respectively.}}
\label{tab:multi_paths}
\begin{scriptsize}
%\begin{small}
\vspace{-1em}
\begin{tabular}{|l|a|b|a|b|}

%\Xhline{2\arrayrulewidth}
\hline \hline
\rowcolor{Gray}
         &\textbf{Multi-HyLSTM} & \begin{tabular}[c]{@{}c@{}}\textbf{HyLSTM}\\ (path embedding)\end{tabular}  & \textbf{BERT}     & \textbf{Multi-BERT} \\ \hline \hline
Acc.(A)   & \textbf{98.99\%} & 95.79\% & 92.49\%     & 95.78\%     \\ \hline
Acc.(K)    &   99.59\%      & \textbf{99.84\%} & 99.48\%   & 96.52\%      \\ \hline
Acc.(U)     &   \textbf{83.02\%}     & 74.44\% & 55.73\%  & 76.07\%     \\ \hline \hline
\end{tabular}
\end{scriptsize}
\vspace{-1.5em}
\end{table}

%The HyLSTM and BERT are two baseline settings that only take one dependence path as input. The HyLSTM here has an extra pretraining phase compared with the HyLSTM in Table~\ref{tab:hylstm}. This is to make the HyLSTM consistent with the BERT, Multi\_LSTM, and Multi\_BERT. 

\noindent
{\sloppy
{\em Multi-path vs. single-path}. Both Multi-HyLSTM and Multi-BERT are more accurate compared with their single-path counterparts. The in-set accuracy is improved from 95.79\% for HyLSTM with single path embedding to 98.99\% for Multi-HyLSTM, and from 92.49\% to 95.78\% for Multi-BERT. More importantly, multi-path aggregation gives significant accuracy improvement for previously unseen cases -- 9.58\% for Multi-HyLSTM and 20.24\% for Multi-BERT.
\par}

%{\bf Ya, just FYI, in the above paragraph, i changed bert to multi\_bert, and hylstm to multi\_hylstm, which i think is easier to understand, as those are the models being discussed, not hylstm and bert.}

\noindent
{\em Improvement from path embedding}. The single-path embedding phase can benefit the API recommendation accuracy, especially for unknown cases. Compared with the basic HyLSTM in Table~\ref{tab:hylstm}, the extra path embedding phase improves the in-set accuracy from 93.00\% to 95.79\%, and from 56.94\% to 76.44\% for unknown cases.  This is likely because the extra path embedding phase exposes the model to the patterns that have not appeared in the task-specific training set.  

\noindent
{\em HyLSTM vs. BERT}. HyLSTM is better at learning programming languages compared with BERT. The HyLSTM outperforms BERT by 3.3\% in-set accuracy improvement and 18.71\% improvement for unknown cases.  The Multi-HyLSTM outperforms Multi-BERT by 3.21\% in-set accuracy improvement and 6.95\% improvement for unknown cases. %That verifies that the code sequences we extracted with program analysis guidance have different requirements with natural language sentences.


\begin{figure}[t]
    \centering
    \includegraphics[width=.99\linewidth]{images/case4.png}
    \vspace{-.5em}
    \caption{\small{Case Study 4. A test case that needs multiple paths to inference correct prediction. The wrong prediction suggested by Path 1 can be fixed after aggregating the influences from two extra paths.}}
    \label{fig:case_study_multi_path}
    \vspace{-2em}
\end{figure}

\noindent
{\em Case Study 4.} The case in Figure~\ref{fig:case_study_multi_path} demonstrates how the multi-path model improves over the single path model. The label \lstinline|Cipher.init(int,Key,AlgorithmParameterSpec)| and  \lstinline|Cipher.init(int,Key)| are indistinguishable, given dependence path 1. Fortunately, paths 2 and 3 provide complementary information to correct it. 


%\smallskip
%\noindent
%\fbox{\begin{minipage}{.99\linewidth}
%The path embedding and the aggregated multi-path vector contribute to a higher accuracy compared with the HyLSTM with the token-level embedding. The path embedding significantly effectively improves the model capability of predicting unseen sequences.  The multi-path form input is more appropriate for code than the common sequential form. The aggregated multi-path vector effectively leverages the useful information from each path to achieve better suggestion. 
%\end{minipage}}

%Data only with slicing:
%When we separate apps with rate 4:1, conduct backward slicing for them. 
%We have 1007681 slices in training set in total!
%48588 of them are unique ones!
%We have 200619 slices in test set in total!
%15126 of them are unique ones!

%When tokenize these slices into token sequence, %we have 764141 sequences in training set and 
%162640 sequences in test set.

% All of them, 54173 sequences are unique

%When we separate apps with rate 9:1, 
%We have 1132309 slices in training set in total!
%51742 of them are unique ones!
%We have 75991 slices in test set in total!
%9158 of them are unique ones!


%After tokenizing into sequences, 
%there are 865691 sequences in training set and 
%61090 sequences in test set.






\smallskip
\noindent
{\bf We summarize our experimental findings as follows:}

\begin{itemize}
   \item Our approach Multi-HyLSTM substantially outperforms the state-of-the-art API recommendation solutions SLANG and Codota in terms of the top-1 accuracy. Multi-HyLSTM achieves an excellent top-1 accuracy of 91.41\% compared with SLANG's 77.44\%. Compared with Codota that achieves a top-1 accuracy of 64.90\% in a manual analysis for 245 test cases, Multi-HyLSTM successfully recommends the 88.98\% cases with the top-1 answer.  
    
    
   
   \item 
    %{\bf Ya, in the sentence below, simplify ``The aggregated multi-path embedding" to ``Our multi-path architecture"? simple name is less confusing}
   
    Our multi-path architecture excels at recognizing new test cases that do not previously appear in the training set. Multi-HyLSTM and Multi-BERT improve the in-set accuracy for unknown cases  by 8.58\% and 20.34\% compared with their single-path counterparts, respectively.
    
    %\item The multi-path architecture works better for program language modeling compared with the sequential architecture. The aggregated multi-path embedding effectively gathers the impacts from multiple dependence paths and generates more accurate suggestions. With the multi-path architecture, Multi-HyLSTM and Multi-BERT improves the \textit{in-set accuracy} of their single-path counterparts from 95.79\% to 98.99\%, and from 92.49\% to 95.78\%, respectively.   
    
   
    %\item 
    %The path embedding contributes the  these only use token-level embedding. The HyLSTM with path embedding has  significant improvement in terms of the inference suggestion accuracy, showing 17.5\% accuracy improvement. With the multi-path embedding aggregation shows further improvement 
   
   \item  HyLSTM with the low-frequency long-range enhancing design outperforms two regular LSTM models. 
   %HyLSTM achieves an optimal trade-off between memorizing capability and inference capability. 
   It improves the inference capability of the LSTM with token-level loss by 13.73\% and the memorizing capability of the LSTM with sequence-level loss by 2.88\%.  
   
   %{\bf Ya, the above paragraph needs to rephrase for several reasons. 1. can you cite the inference capability number 13.73\% like you did in the intro, instead of 2.23\% and 2.38\% (just remove those 2 numbers, no need), as that inference number is more important? 2. the last sentence "without hurting..." sounds a bit negative and causes confusion, rephrase}
    
    %\item Transitive labeling (used in \textit{sDep2vec}) is more effective at differentiating insecure and secure code than neighbor-based labeling (used in \textit{dep2vec}). For misuse detection (task~3), \textit{sDep2vec}'s accuracy is 14\% higher than \textit{dep2vec}'s. However, the task-specific one-hot encoding, involving 15X  parameters, is 5\% more accurate than \textit{sDep2vec}.  

    
    \item {\sloppy Program analysis guidance significantly improves the quality of code embedding and the recommendation accuracy. Enabled by these techniques, \textit{dep2vec} outperforms \textit{byte2vec} by 36\% for the next API recommendation, and 45\% for API sequence recommendation. \par}
    
    
    Similarly, the interprocedural slicing and API dependence graph construction also benefit in substantial accuracy improvements (31\% for the next API recommendation task and 39\% for the next API sequence recommendation task, respectively) even without embedding. 
    
    
    %We made a substantial effort to interpret neural network results and compare model capabilities by conducting time-consuming manual case studies. 
%
% Daphne commented below out due to space.
%Case 1 explains how program analysis preprocessing simplifies the code suggestion task by solving the code entanglement.  Case 2 confirms the advantages of token embeddings in recognizing new previously unseen tokens and make inferences. Case 4 verifies the benefits of enhancing the low frequent long-range influences in improving the code suggestion accuracy.   
%
%We are in the process of publishing our datasets as an accuracy benchmark.

\end{itemize}


\smallskip
\noindent
{\em Performance and runtime.} With the distributed training of 8 workers, our training time is significantly improved. Most of our experiments are completed within 5 hours. We noticed that when the \textit{dep2vec} embedding is applied, the training becomes much faster than the one-hot encoding, improved from around 5 hours to 2 hours. 
%{\bf Ya, if we don't have runtime data, then at least comment on the general range of runtime of various operations. Otherwise, the reviewers will complain. thanks.}





\section{Threats to Validity and Limitations}

\noindent
{\bf Threats to Validity.}
A threat to internal validity is that the next token of a given sequence may not be the only choice. It may cause the prediction accuracy to be misaligned with the model capability. To avoid this issue, we collect a reasonable next token set to calculate accuracy. Although this set may not be complete, it reflects all the possibilities seen in the training phase. We think it is reasonable to evaluate the model according to the unseen knowledge rather than the full knowledge.    
%
Another threat to external validity is that our dataset is highly repetitive, which is different from other domains like images.  However, it is the characteristics of the code sequences. Different source code sequences may become identical after program analysis, which is expected. 

\noindent
{\bf Limitations.}
{\sloppy
\noindent
Our threat model described in Section~\ref{sec:challenges} can be further expanded to include other Java security libraries (e.g., Java Spring framework) and vulnerability types (e.g., TLS/SSL authentication-related vulnerabilities). We expect our pre-processing, embedding, and suggestion methodologies  to apply to these new scenarios.   
%
%
It is well known that static analysis tends to overestimate execution paths. Thus, the slices and dependence paths used for training embeddings and making suggestions might not necessarily occur. However, the infeasible paths appear together with the realizable paths. Our Multi-HyLSTM model can still make correct predictions, as it is decided by multiple data-flow paths. We expect the deep learning model to automatically learn which path to trust by training.
%{\bf Ya, the last sentence seems to be a big claim -- so the multipath model is immune to the static program analysis limitation? please explain a bit more.}
%
The dependence paths extracted from API dependence graphs may be incomplete, as we omit recursions in the call stacks and in the node paths. We also terminate the path when the depth of call stacks is beyond~10. A previous study experimentally showed the impact of limited depth exploration to be negligible in practice~\cite{rahaman2019cryptoguard}. %{\bf Ya, cite sazzadur's ccs cryptoguard paper.} 

% Daphne commented sentence below out, as it sounds rather arbitrary and subjective...
% because they are only corner cases and our approach makes suggestion based on several rather than all paths. 
%
%
%These pre-processing issues may lead to inaccurate or incomplete embedding training, as well as errors in downstream tasks. {\bf Ya, need a few sentences commenting on how this limitation impacts your accuracy. how likely this limitation could occur. Currently, you make it sound pretty serious, invalidating your prediction. also how to fix it?}
\par}


==> Comprehensive Comparisons of Code Embedding Methodologies for Java Cryptographic Applicatons/Sections/6-related_work.tex <==

\section{Other Related Work}

%\sloppy{
%\noindent
%\textit{Code repair without neural networks.} Several studies demonstrated how to automatically detect and repair cryptographic API misuses based on manually generated patterns~\cite{ma2016cdrep,ma2017vurle,kim2013automatic}. Although highly effective, these approaches require manual pattern-generation efforts for new vulnerabilities.
%Genetic programming-based approaches~\cite{le2012genprog,le2012systematic} automatically generate patches from code mutations and verify them against test suites. Accuracy in recognizing previously unseen cases remains an unsolved challenge for these non-neural-network based approaches~\cite{long2016analysis}. 
%\par}

\noindent
\textit{Code completion work.} Many studies validated the naturalness of code sequences~\cite{hindle2012naturalness,tu2014localness,ray2016naturalness,hindle2016naturalness,allamanis2018survey,rahman2019natural}, which inspires a line of work to build language models for code completion/suggestion tasks~\cite{campbell2014syntax,bhatia2016automated,santos2018syntax,bhatia2018neuro,tufano2020generating,svyatkovskiy2020intellicode}.
%
%{\bf Ya, please write RNN out in full name above, if first appearance. thanks.}
%
For example, Campbell {\it et al.}~\cite{campbell2014syntax} utilized the $n$-gram model trained on the code tokens to localize and give suggestions for Java syntax error correction. Bhatia \textit{et al.}~\cite{bhatia2016automated,bhatia2018neuro} trained the Recurrent Neural Networks (RNN) on the student programming assignments to solve syntax errors in C++ by replacing or inserting suggested code tokens. Recently, a more advanced and powerful model, Transformer~\cite{vaswani2017attention}, is also applied to code generation tasks in ~\cite{svyatkovskiy2020intellicode,tufano2020generating}.  
%Gupta {\it et al.} learned the mapping from typographic errors (e.g. missing a semicolon) in student C programming assignments to corresponding fixes with supervised learning~\cite{gupta2017deepfix} and deep reinforcement learning~\cite{gupta2018deep}, respectively. 
These studies are built on top of the general source code token sequences or AST paths to solve syntax problems. However, as pointed in ~\cite{hellendoorn2017deep}, there do exist many program specific challenges that hinder the naive application of the language models borrowed from natural language processing domain. 
%Authors in~\cite{harer2018learning} enabled the application of Generative Adversarial Neural Networks (GAN) in code repair problems by fixing several domain-specific challenges (e.g., non-differentiable discrete data, lacking bijection guarantee). Although GAN has the advantage of not requiring pairwise data, its accuracy results are upper bounded by the LSTM based model according to \cite{harer2018learning}.  %the main applications considered in~\cite{harer2018learning} are not related to security. The changed code is evaluated by blue scores, which are typically used in NLP for assessing text quality. 

 Some studies focus on completion for API methods to improve the productivity of developers and solve API related problems~\cite{raychev2014code,nguyen2013statistical,nguyen2016api,nguyen2016learning}. Program analysis techniques are often applied to extract API sequences from source code to build language models. Nguyen \textit{et al.} presented a graph representation of object usage model (GORUM) to represent interactions between different objects and associated methods~\cite{nguyen2009graph}. They built Hidden Markov models for the state of objects and predict methods~\cite{nguyen2013statistical,nguyen2016learning}. However, these methods may require to build endless Markov models for different object types. Raychev \textit{et al.}~\cite{raychev2014code} built RNN and n-gram models on top of the object histories defined by themselves for API method recommendation. The object histories consist of the method call events in the temporal order. Although its top-16 accuracy (96.43\%) is pretty good, it only achieves a top-1 accuracy of 69.05\%.           

\noindent
{\em Code embedding work}.
Code embeddings (e.g.,~\cite{alon2019code2vec,henkel2018code,allamanis2015suggesting}) that automatically learn the vector representations of code tokens, have shown great improvement on the learning accuracy. There are multiple task-specific embedding studies (e.g., \cite{zhao2018deepsim,xu2017neural,alon2019code2vec,allamanis2015suggesting,li2018vuldeepecker}) which train the embedding jointly with the downstream task.  For example, Zhao {\it et al.}~\cite{zhao2018deepsim} trained embeddings of code snippets with the code similarity detection. 
Alon {\it et al.}~\cite{alon2019code2vec} designed a path-based attention network to train the code snippet embedding and predict its semantic tag (e.g., method name, class name). 
 %Xu et al. \cite{xu2017neural} embed binary functions from the attributed control flow graphs (ACFG) to detect code similarity across platforms. 
 %Li {\it et al.} \cite{li2018vuldeepecker} decomposed software into code gadgets and embedded them into vectors for vulnerability detection.  
As these code vectors are optimized for specific tasks, they cannot be directly used in our API recommendation setting. 


%General-purpose embedding, the focus of our work, is pre-trained without downstream tasks. Thus, they are independent of downstream tasks. There are two types of general-purpose embeddings, the static embedding for every single tokens and the contextualized embedding along with the language models.


% Eberhardt et al.~\cite{eberhardt2019unsupervised} learn the probabilistic model based on APIs to mine the aliasing specifications to help the pointer-to analysis~\cite{eberhardt2019unsupervised}. 

%\subsection{Contextualized Embedding}

%Manual code generation is error-prone and causes vulnerabilities \cite{meng2018secure}. Although common vulnerabilities are relatively easy to fix (e.g., 2.6 minutes for removing dead code, 6.9 minutes for the lack of authorization check \cite{cornell2012}), complex ones take much longer (e.g., SQL injection requires 97.5 minutes \cite{cornell2012}). 

%Existing automatic code generation research is still in its infancy. 




  

%It also cannot handle new code snippets with unseen paths. In addition, since the network is trained with semantic tags (i.e. names of methods, classes and projects) as supervision, it is unclear its extensibility for new code snippets out of the training semantic tags.

 Regardless of the downstream tasks, general-purpose embeddings are trained in the unsupervised way, e.g.,~\cite{nguyen2017exploring,harer2018automated}. The general-purpose embedding of source code in \cite{harer2018automated} improves the results of vulnerability detection compared with manual defined features. Recently, several embedding solutions for low-level code were  reported~\cite{ding2019asm2vec,ben2018neural}. Asm2Vec~\cite{ding2019asm2vec} embedded assembly functions based on their control flow graphs and apply embedding vectors for similarity detection between binaries. The authors in \cite{ben2018neural} learned embeddings for LLVM IR instructions and used it for algorithm classification and device mapping decisions (e.g., CPU vs. GPU). 
 %In \cite{white2019sorting}, White et al. leverage the similarity of code embeddings to optimize patch searching  in traditional code repair systems~\cite{le2012genprog,long2015staged}. 
However, these designs for embedding source code tokens, low-level instructions, or LLVM IRs cannot be directly applied to API elements. 

\noindent
{\em Other API learning work.}
There is a line of work designed to solve API-related tasks~\cite{nguyen2016mapping,gu2016deep,nguyen2017exploring,chen2019mining,eberhardt2019unsupervised,bavishi2019autopandas,bui2019sar,xie2020api}. 
%{\bf Ya, what is API learning? i feel our work is vaguely also API learning, so confusing, as readers may wonder can these solutions used by us? please explain, so readers can tell the differences.} 
Nguyen {\it et al.}~\cite{nguyen2017exploring,nguyen2016mapping} mapped the semantic similar JDK APIs with .NET APIs through their similar embedding vectors. Chen {\it et al.}~\cite{chen2019mining} trained the API embedding based on the API description (name and documents)  and usage semantics to infer the likely analogical APIs between third party libraries. 
%Bui {\it et al.}~\cite{bui2019sar} minimized the manual effort for code corpus preparation in the cross language API migration by introducing GAN to align the API embeddings across language. 
%Gu {\it et al.}~\cite{gu2016deep} trained the RNN-based Encoder-Decoder model with the API embedding to translate between natural language sentences and API sequences. 
However, these solutions aimed at applying embeddings to help map analogical APIs, which is different from our API recommendation task with a high accuracy requirement. %\bimal{rephrase last sentence. what does ``rough semantics'' mean? a verb is missing i think.} %many functionally similar APIs.% Our work also focuses on learning the API usage and embedding. However, 
%
% Daphne commented below sentence out, as it's not very related it seems, rephrase later?
%For our task with high accuracy requirement, it is unclear that how much these API embedding approaches can help. In addition, our main research focus is on comparing various methodologies and model designs to achieve the high suggestion accuracy. 
%
%
%To remove noises in code, several pre-processing approaches have been proposed. For example, \cite{henkel2018code} performed intra-procedural symbolic execution first and trained embedding vectors of symbolic abstractions from symbolic traces. \cite{allamanis2018learning} constructed graph-based representations for code and applied the Gated Graph Neural Networks (GGNN) to embed graph nodes.   \cite{allamanis2017learning} learned embeddings for symbolic expressions including algebraic and logical expressions. Their embedding network is trained to represent semantic equivalence of expressions, i.e., equivalent expressions are represented as close vectors even when they are syntactically different.  Unlike our work, these solutions are not specifically designed for security applications. Thus, it is unclear how well these embeddings perform in terms of prediction and detection accuracy. 

%These embeddings are  general-purpose, as they are not trained with any downstream applications. These embedding studies on low-level code complement our work on embedding high-level APIs\footnote{As APIs and constants are shared across all programs, our work does not have the out-of-vocabulary problem.}.


%\cite{kolosnjaji2016deep} applies Neural networks to malware detection. It uses system call sequences as detected objects and constructs a convolutional and recurrent neural network to improve the performance.


%Current deep-learning-based software solutions can be divided into 3 categories in terms of code embedding. First, one-hot encoding every token in programming code. Second, directly to borrow word2vec method into the source code. Third, applying word2vec on some intermediate representations of code (e.g. AST, CFG). All of these methods are still quite limited. 

%{\em Symbolic representation}
    %Several researches treats a program as a composition of tokens %\cite{allamanis2014learning,allamanis2015suggesting,allamanis2013mining}. Every token is indexed as a feature. These token feature based representations are input to corresponding training models.% There are two major limitations of these approaches in SE domain. First, the tokens in source codebase are unbounded. There is no way to deal with a unseen token that is very likely to appear in the test or application stages. Second, the structural information of the program is totally lost when directly migrate NLP deep learning solutions to programming language domain.  
    
    %\item \textit{Task-specific Embedding.}
    %There are also some work realize that an efficient embedding learning are beneficial to the final efficiency as well as the precision of the neural networks \textcolor{red}{citation}. 
    %\item \textit{General Embedding.}
    

%There are three categories for code embedding.
%\subsection{Symbolic Representation}

%\subsection{Single-purpose Embedding}

%\subsection{General-purpose Embedding}


%One of the crucial challenges met by AI in software systems is the shift in the development paradigm induced by ML and AI\cite{khomh2018software}. Specifically, the rules of the program code need to be learned from training data. 






%{\it Vulnerability Detection and Repair with Traditional Approaches}

%\cite{pham2010detection} conducted an empirical study on thousands of vulnerabilities and found most of them are due to code reuse. They developed a tool called SecureSync, which detect vulnerabilities by calculating the similarity score of ASTs.

%\cite{le2019automated} summarizes the state-of-the-arts bug repair techniques in two categories, heuristic repair and constraint-based repair. These techniques work through searching over a space of changes to the input source code. These techniques can also be enhanced by machine learning, which we call learning-aided repair.

%Genetic Programming-based approaches \cite{le2012genprog} repair a buggy program by mutating a statement by a deletion, an insertion (another statement in the same program), or a swap with another statement. The mutation is evaluated by a test suite. Kim et al \cite{kim2013automatic} improved the Genetic Programming by manually define several common fix patterns by inspecting more than 60,000 human-written patches. Instead of random mutation, the fix patterns are used as the patch search space.  However, Rinard ea al \cite{long2016analysis} point out that the naive searching of the patch spaces is more likely to generate plausible patches rather than correct patches.


%Ma et al. manually studied the vulnerabilities types and their corresponding fix patterns \cite{ma2016cdrep}. They further automatically extracted context pattern of vulnerabilities and edit patterns to fix them by the vulnerabilities and their fix examples \cite{ma2017vurle}. It works on AST level.
 
%Murali et al. \cite{murali2017bayesian} applies language model to API sequence and achieves to detect abnormal API sequence occurence in codebase. 

%Rinard et al. develop a Staged Program Repair \cite{long2015staged} which is based on the condition synthesis technique. It efficiently reduce the patch search space by some parameterized transformation patterns. Based on this traditional approach as a baseline, they also develop a new tool \cite{long2016automatic} which uses machine learning techniques to learn from past successful human patches to rank the possibility for the patches in the patch search space. They also designs some code inference algorithms\cite{long2017automatic,rinard2018active} to regenerate code from existing codebase.

%\cite{zhang2018neural} uses a neural model to guide the conventional Programming By Example (PBE) problems in program synthesizing. 

%{\it Programming Language Processing with Deep Learning-based Approaches}
%Hindle et al \cite{hindle2012naturalness} first investigate the naturalness of software and answer the question that software language also maintain naturalness like the natural language so that it can also be handled by the statistical model. After that Ray et al \cite{ray2016naturalness} argues that buggy code also has naturalness so that it is promising to solve bug-related tasks with statistical models.



%{\it Other tasks with big code}

%Some big code research directly applies the statistical language model of the natural language to the programming language. Allamanis et al firstly build a giga-token probabilistic language model of source code \cite{allamanis2013mining}. It applies the n-gram model on 352 million lines of Java code. It analyzes some complexity metrics of the codebase in the token level. Then, they also applies the language model to the code convention learning task\cite{allamanis2015suggesting}. Specifically, the learned language model works for suggesting names for identifiers. Besides variable naming task, method and class naming tasks are also explored in \cite{allamanis2015suggesting}. Raychev et al \cite{raychev2014code} extract method calls sequence from a large codebase as sentences with static analysis. Then, they apply the statistical language models to these sentence. The learned statistical model is used to achieve code completion. That is, suggesting the correct API for a sentence with a missing API. \cite{raychev2015predicting} builds a dependency network from known properties (e.g. constant and APIs) to unknown properties (e.g. variable names). It applies a graphical models to learn from mined dependency networks and achieves the tasks (i) predicting names of local variables and (ii) predicting type annotations of function arguments for JavaScript. 



%\cite{zuo2018neural} applies neural translation model in NLP to large-scale binary code and achieves to identify code similarity.

%\cite{ling2019deepsec} explores the adversarial examples to evaluate the reliability of deep learning models.
%\cite{paletov2018inferring} infers Crypto API Rules from code changes.






==> Comprehensive Comparisons of Code Embedding Methodologies for Java Cryptographic Applicatons/Sections/7-conclusions_and_future_work.tex <==

%\vspace{-1em}
\section{Conclusions}

Data-driven code suggestion approaches need to be deeply integrated with program-specific techniques, as code and natural languages have fundamentally different characteristics.
%
We proposed new code suggestion techniques for securing Java cryptographic API usage, and comprehensively compared
our approach with a variety of state-of-the-arts and intermediate solutions. 
Our extensive evaluations with API recommendation and API sequence recommendation tasks demonstrated that our approach is more appropriate for programming languages than common sequential models designed for natural languages. 
%Our extensive evaluations with API recommendation and API sequence recommendation tasks demonstrated that the multi-path architecture is more appropriate for programming languages than common sequential models designed for natural languages. 


%We systematically and comprehensively compared a number of code suggestion methodologies for securing Java cryptographic API usage. We performed extensive experimental evaluations with code token suggestion and code sequence suggestion tasks and demonstrated that the multi-path architecture is more appropriate for code suggestion than common sequential architectures designed for natural languages. 

%Daphne commented below out due to space
%We discussed the program-specific global influence issue and introduced the  hybrid loss to improve it. We also conducted multiple in-depth case studies to identify the reasons behind the misclassified neural network results, which are notoriously difficult to explain. Besides the security insights, our work also produced several large Android-based embedding training datasets, which we will publish. 

% Daphne commented below out due to space
% The program-specific characteristics revealed in our work pointed out several promising future directions, including new architecture designed for program language model and program-analysis guided learning solutions.  

% add to limitations
%One limitation of our work is the sound but not complete data caused by static program analysis.  


%Our case studies on false positive and false negative cases pointed out several promising future directions, including adding weights to tokens with advanced neural network architectures and mechanisms to further highlight security semantics (i.e., secure vs. insecure) in embedding training beyond programming semantics (e.g., API sequences).


%There are a couple of open problems that can be explored in the future. First, what are most significant features used for security classification tasks? The current features (i.e., all tokens the sequence has) seem to be insufficient to recognize secure sequences and long insecure sequences. It would be better if stronger indicators (e.g., what the sequence does not have) could be included as features. Second, how to train embeddings for downstream task that requires features beyond semantics? The pre-trained embedding has a goal to capture semantics into vectors. However, in security classification tasks, some of the similar vector pairs do harm to these tasks while some of them still benefit. How to pinpoint and avoid the undesired similar code vectors is an interesting future work.    Finally, the data quality is always crucial to final results. The statistical bias of features may result in misprediction. How to measure and improve the quality  of a dataset is worth further exploration.  

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)
